CoWeave: Identity-Specific Context Reasoning for Persistent Multi-Camera Tracking

Multi-camera tracking must associate each cross-camera arrival with an identity and preserve that identity in memory. Two coupled failures undermine this process: shared context can support competing identity assignments equally, and incorrect memory attribution can propagate errors to later arrivals. We propose CoWeave, which unifies assignment scoring, evidence retrieval, and memory maintenance through a common identity decision loss. Candidate-conditioned scoring compares joint assignments using evidence that distinguishes them and allows unresolved outputs when committing is too costly. A budgeted reader selects historical sources by their predicted reduction in decision loss, sharing each source across active people without duplicate access. Memory stores each observation with revisable identity ownership and separately tracks the validity of its relations. On MTMMC, under a common causal stream and budget, CoWeave improves global identification F1 from 72.9 to 80.5 over causal GMT and reduces wrong arrivals from 5.9% to 2.5%. Among arrivals with 30 subsequent observations, the fraction remaining correct from arrival throughout follow-up rises from 67.0% to 82.1%. Gains also hold with each method's native front end and on WILDTRACK, MMPTrack, and DIVOTrack.

==> figures/tikz/coweave_style.tex <==
\providecommand{\cwStyleLoaded}{}
\definecolor{cwA}{HTML}{5FB8C2}      % identity A, teal (fills, bars)
\definecolor{cwB}{HTML}{F2A0C8}      % identity B, rose (fills, bars)
\definecolor{cwC}{HTML}{B4A7D6}      % identity C
\definecolor{cwAd}{HTML}{1A7F8E}     % identity A, strokes and letters (4.6:1 on white)
\definecolor{cwBd}{HTML}{B8418A}     % identity B, strokes and letters (5.0:1 on white); magenta side, apart from the coral error red
\definecolor{cwCd}{HTML}{7A6AB5}
\definecolor{cwOK}{HTML}{548235}     % correct (glyphs)
\definecolor{cwBad}{HTML}{D36265}    % wrong (glyphs, the focal error line)
\definecolor{cwGray}{HTML}{6B6B6B}   % new / unresolved / unknown (strokes, text)
\definecolor{cwInk}{HTML}{222222}
\definecolor{cwNote}{HTML}{5A5A5A}   % secondary text (6.9:1 on white)
\definecolor{cwPanel}{HTML}{F1F3F4}  % the CoWeave band only
\definecolor{cwRule}{HTML}{8F999F}   % dividers (3.0:1 on white)
\definecolor{cwHair}{HTML}{C9CFD3}   % panel separators
\definecolor{cwYel}{HTML}{F0E442}    % annotated person in observed-output figures
\tikzset{
  cw/.style={x=1pt,y=1pt,line cap=round,line join=round,font=\scriptsize,text=cwInk},
  panel/.style={fill=none,draw=none},
  ptitle/.style={anchor=north west,inner sep=0pt,font=\footnotesize\bfseries},
  psub/.style={anchor=north west,inner sep=0pt,font=\scriptsize,text=cwNote},
  plab/.style={inner sep=0pt,font=\scriptsize},
  phead/.style={inner sep=0pt,font=\scriptsize\bfseries},
  pnote/.style={inner sep=0pt,font=\scriptsize\itshape,text=cwNote},
  idn/.style={circle,draw=#1d,line width=0.6pt,shading=radial,inner color=white,outer color=#1!42,minimum size=11.5pt,inner sep=0pt,font=\scriptsize\bfseries,text=#1d!80!black},
  obs/.style={circle,draw=cwInk!75,line width=0.5pt,fill=white,minimum size=11.5pt,inner sep=0pt,font=\scriptsize},
  out/.style={rounded corners=2.5pt,draw=#1d,line width=0.8pt,fill=#1!16,minimum height=10.5pt,minimum width=15pt,inner sep=1.5pt,font=\scriptsize\bfseries,text=#1d},
  newid/.style={rounded corners=2.5pt,draw=cwGray,line width=0.5pt,fill=white,minimum height=10.5pt,minimum width=15pt,inner sep=1.5pt,font=\scriptsize\itshape,text=cwGray},
  unres/.style={rounded corners=2.5pt,draw=cwGray,dash pattern=on 1.6pt off 1.2pt,line width=0.6pt,fill=white,minimum height=10.5pt,minimum width=15pt,inner sep=1.5pt,font=\scriptsize,text=cwGray},
  ctx/.style={draw=cwInk!70,line width=0.5pt,dash pattern=on 2pt off 1.5pt},
  link/.style={draw=cwInk!80,line width=0.8pt},
  cand/.style={draw=cwInk!55,line width=0.5pt},
  flow/.style={draw=cwInk,line width=0.8pt,-{Stealth[length=4pt,width=3.4pt]}},
  thin/.style={draw=cwInk,line width=0.5pt,-{Stealth[length=3pt,width=2.6pt]}},
  tag/.style={fill=white,draw=cwInk!70,line width=0.5pt,inner sep=1pt,font=\scriptsize\bfseries},
  photo/.style={inner sep=0pt,draw=cwInk!45,line width=0.5pt},
  okmark/.style={text=cwOK,font=\footnotesize\bfseries,inner sep=0pt},
  badmark/.style={text=cwBad,font=\footnotesize\bfseries,inner sep=0pt},
  oursband/.style={fill=cwPanel,draw=none},
  hair/.style={draw=cwHair,line width=0.5pt},
}
\newcommand{\cwok}{\ensuremath{\checkmark}}
\newcommand{\cwbad}{\ensuremath{\boldsymbol{\times}}}
\newcommand{\cwown}[6]{%
  \pgfmathsetmacro{\cwoa}{#3*#5}\pgfmathsetmacro{\cwob}{#3*#6}%
  \fill[cwA!80] (#1,#2) rectangle ++(\cwoa,#4);
  \fill[cwB!80] (#1+\cwoa,#2) rectangle ++(\cwob,#4);
  \fill[cwGray!25] (#1+\cwoa+\cwob,#2) rectangle (#1+#3,#2+#4);
  \draw[cwInk!60,line width=0.5pt] (#1,#2) rectangle ++(#3,#4);}
\newcommand{\cwphoto}[7]{\node[photo,anchor=#7] (#1) at (#2,#3) {\includegraphics[width=#4pt,height=#5pt]{figures/tikz/assets/cw/#6}};}
\newcommand{\cwgt}[3]{%
  \edef\cwtmp{\csname cwbox@#2\endcsname}%
  \expandafter\cwgtbody\cwtmp\relax{#1}{#3}}
\def\cwgtbody#1/#2/#3/#4\relax#5#6{%
  \path let \p1=(#5.south west), \p2=(#5.north east) in
    coordinate (cwgt-sw) at ({\x1+#1*(\x2-\x1)},{\y1+#2*(\y2-\y1)})
    coordinate (cwgt-ne) at ({\x1+#3*(\x2-\x1)},{\y1+#4*(\y2-\y1)});
  \draw[#6] (cwgt-sw) rectangle (cwgt-ne);}
\newcommand{\cwfeat}[5]{%
  \foreach \cwv [count=\cwi from 0] in {#5}{\fill[cwInk!\cwv] (#1+\cwi*#3,#2) rectangle ++(#3,#4);}
  \foreach \cwv [count=\cwi from 1] in {#5}{\xdef\cwn{\cwi}}%
  \draw[cwInk!60,line width=0.5pt] (#1,#2) rectangle ++(\cwn*#3,#4);}
\newcommand{\cwmat}[8]{%
  \fill[cwSup!#4] (#1,#2) rectangle ++(#3,#3);   \fill[cwSup!#5] (#1+#3,#2) rectangle ++(#3,#3);
  \fill[cwSup!#6] (#1,#2-#3) rectangle ++(#3,#3); \fill[cwSup!#7] (#1+#3,#2-#3) rectangle ++(#3,#3);
  \draw[cwInk!60,line width=0.5pt] (#1,#2-#3) rectangle ++(2*#3,2*#3) (#1+#3,#2-#3) -- ++(0,2*#3) (#1,#2) -- ++(2*#3,0);
  \ifnum#8>0
    \node[plab,anchor=south,font=\scriptsize\bfseries,text=cwAd] at (#1+0.5*#3,#2+#3+0.5) {A};
    \node[plab,anchor=south,font=\scriptsize\bfseries,text=cwBd] at (#1+1.5*#3,#2+#3+0.5) {B};\fi
  \ifnum#8=1
    \node[plab,anchor=east] at (#1-1,#2+0.5*#3) {$x$};
    \node[plab,anchor=east] at (#1-1,#2-0.5*#3) {$y$};
  \fi}
\tikzset{cam/.pic={
  \path[fill=cwInk!80,rounded corners=0.5pt] (-3.5,-1.6) rectangle (0.9,1.6);
  \path[fill=cwInk!80] (0.9,-0.4) -- (3.5,-1.7) -- (3.5,1.7) -- (0.9,0.4) -- cycle;}}
\newcommand{\cwfov}[6]{%
  \fill[cwInk!10] (#1,#2) -- ++(#3-28:#4) arc[start angle=#3-28,end angle=#3+28,radius=#4] -- cycle;
  \draw[cwInk!35,line width=0.5pt] (#1,#2) -- ++(#3-28:#4) (#1,#2) -- ++(#3+28:#4);
  \pic[rotate=#3] at (#1,#2) {cam};
  \node[plab,font=\scriptsize\bfseries,anchor=#6,outer sep=5pt] at (#1,#2) {#5};}
\newcommand{\cwcam}[2]{%
  \path[fill=cwInk!80,rounded corners=0.6pt] (#1,#2-2.2) rectangle ++(5.6,4.4);
  \path[fill=cwInk!80] (#1+5.6,#2-0.6) -- (#1+8.6,#2-2.2) -- (#1+8.6,#2+2.2) -- (#1+5.6,#2+0.6) -- cycle;}
\newcommand{\cwlock}[2]{%
  \draw[cwInk,line width=0.6pt] (#1-1.6,#2+1.2) -- (#1-1.6,#2+2.6) arc[start angle=180,end angle=0,radius=1.6pt] -- (#1+1.6,#2+1.2);
  \path[fill=white,draw=cwInk,line width=0.6pt,rounded corners=0.5pt] (#1-2.6,#2-2.4) rectangle (#1+2.6,#2+1.4);}
\newcommand{\cwenc}[6]{%
  \path[fill=cwInk!8,draw=cwInk!70,line width=0.6pt,rounded corners=1pt] (#2,#3-#5/2) -- (#2+#4,#3-#6/2) -- (#2+#4,#3+#6/2) -- (#2,#3+#5/2) -- cycle;
  \coordinate (#1-in) at (#2,#3); \coordinate (#1-out) at (#2+#4,#3);}
\definecolor{cwTAmber}{HTML}{FFF1CC} \definecolor{cwLAmber}{HTML}{E2B33C} \definecolor{cwHAmber}{HTML}{FFE699}
\definecolor{cwTGrey}{HTML}{F3F7F9}  \definecolor{cwLGrey}{HTML}{899FA5}  \definecolor{cwHGrey}{HTML}{C4D4DD}
\definecolor{cwTRose}{HTML}{FDF0F3}  \definecolor{cwLRose}{HTML}{D99AB3}  \definecolor{cwHRose}{HTML}{FBDCE0}
\definecolor{cwTGreen}{HTML}{E8F3E2} \definecolor{cwLGreen}{HTML}{8DBF6E}  \definecolor{cwHGreen}{HTML}{C7E4B3}
\definecolor{cwTBad}{HTML}{FDF0F3}   \definecolor{cwLBad}{HTML}{D36265}   \definecolor{cwHBad}{HTML}{FBDCE0}
\definecolor{cwTGood}{HTML}{E8F3E2}  \definecolor{cwLGood}{HTML}{8DBF6E}  \definecolor{cwHGood}{HTML}{C7E4B3}
\definecolor{cwHi}{HTML}{FFE699}     \definecolor{cwHiD}{HTML}{BF9000}    % key-claim highlight (yellow)
\definecolor{cwSup}{HTML}{8C8CE0}    \definecolor{cwSupL}{HTML}{CECEFA}   % support / score (lavender ramp)
\definecolor{cwTokA}{HTML}{99CCFF} \definecolor{cwTokB}{HTML}{C7E4B3} \definecolor{cwTokC}{HTML}{FFE699} \definecolor{cwTokD}{HTML}{CECEFA}
\definecolor{cwTSky}{HTML}{E4F6FC} \definecolor{cwLSky}{HTML}{9DC3E6} \definecolor{cwHSky}{HTML}{DDEAF7}
\definecolor{cwGold}{HTML}{FFC000} \definecolor{cwGoldL}{HTML}{FFF1C9} \definecolor{cwPeach}{HTML}{F8CAAC}
\definecolor{cwGlass}{HTML}{E4F6FC} \definecolor{cwGlassL}{HTML}{A8CFE8}
\definecolor{cwFeat}{HTML}{55636F}
\newcommand{\cwbadge}[1]{\tikz[baseline=-0.62ex]\node[circle,fill=cwInk,text=white,inner sep=0pt,minimum size=8.4pt,font=\scriptsize\bfseries] {#1};}
\newcommand{\cwbox}[7]{%
  \path[fill=cwT#5,draw=cwL#5,line width=0.75pt,dash pattern=on 2.6pt off 1.7pt,rounded corners=4pt] (#1,#2) rectangle (#3,#4);
  \node[anchor=west,inner sep=0pt,font=\footnotesize\bfseries\itshape,text=cwInk] at (#1+4,#4-7.2) {\cwbadge{#6}\,\,#7};}
\newcommand{\cwtab}[6]{%
  \path[fill=cwH#5,draw=cwL#5,line width=0.6pt,rounded corners=3pt] (#1,#2) rectangle (#3,#4);
  \node[align=center,inner sep=0pt,font=\scriptsize\bfseries,text=cwInk] at ({(#1+#3)/2},{(#2+#4)/2}) {#6};}
\newcommand{\cwplate}[5]{%
  \path[fill=cwL#5!70,rounded corners=1pt] (#1,#3-#4/2-1.6) -- (#2,#3-#4/2-1.6) -- (#2+7,#3+#4/2-1.6) -- (#1+7,#3+#4/2-1.6) -- cycle;
  \path[fill=cwH#5,draw=cwL#5,line width=0.5pt,rounded corners=1pt] (#1,#3-#4/2) -- (#2,#3-#4/2) -- (#2+7,#3+#4/2) -- (#1+7,#3+#4/2) -- cycle;}
\newcommand{\cwtok}[5]{%
  \foreach \cwi in {1,...,#3}{\foreach \cwj in {1,...,#4}{
    \pgfmathtruncatemacro{\cwlv}{mod(\cwi*37+\cwj*53,50)+12}
    \pgfmathtruncatemacro{\cwtk}{mod(\cwi+2*\cwj,4)}%
    \ifcase\cwtk\def\cwtc{cwTokA}\or\def\cwtc{cwTokB}\or\def\cwtc{cwTokC}\else\def\cwtc{cwTokD}\fi
    \path[fill=\cwtc,draw=cwInk!55,line width=0.35pt] (#1+\cwi*#5-#5,#2-\cwj*#5) rectangle ++(#5,#5);}}
  \draw[cwInk!70,line width=0.5pt] (#1,#2-#4*#5) rectangle (#1+#3*#5,#2);}
\newcommand{\cwfilm}[4]{%
  \path[fill=cwInk!88,rounded corners=1.5pt] (#1,#2) rectangle (#3,#4);
  \pgfmathsetmacro{\cwfn}{floor((#3-#1-4)/6)}
  \foreach \cwk in {0,...,\cwfn}{\path[fill=white] (#1+3+\cwk*6,#2+1.1) rectangle ++(2.6,1.9);
    \path[fill=white] (#1+3+\cwk*6,#4-3) rectangle ++(2.6,1.9);}}
\tikzset{pill/.style={fill=cwGoldL,draw=cwHiD,line width=0.5pt,rounded corners=3pt,inner xsep=3pt,inner ysep=1.6pt,font=\scriptsize\itshape}}
\def\cwdx{0.55}\def\cwdy{0.42}
\newcommand{\cwslab}[6]{%
  \colorlet{cwslabt}{#5}\colorlet{cwslabe}{#6}%
  \pgfmathsetmacro{\cwsx}{#4*\cwdx}\pgfmathsetmacro{\cwsy}{#4*\cwdy}%
  \path[fill=cwslabe!55,blur shadow={shadow blur steps=6,shadow xshift=1.2pt,shadow yshift=-1.6pt,shadow opacity=25}]
     (#1,#2-3) -- (#1+#3,#2-3) -- (#1+#3+\cwsx,#2+\cwsy-3) -- (#1+#3+\cwsx,#2+\cwsy) -- (#1+\cwsx,#2+\cwsy) -- (#1,#2) -- cycle;
  \path[fill=cwslabe!70] (#1,#2-3) rectangle (#1+#3,#2);
  \path[fill=cwslabe!45] (#1+#3,#2-3) -- (#1+#3+\cwsx,#2+\cwsy-3) -- (#1+#3+\cwsx,#2+\cwsy) -- (#1+#3,#2) -- cycle;
  \path[top color=cwslabt!55,bottom color=cwslabt,draw=cwslabe,line width=0.5pt]
     (#1,#2) -- (#1+#3,#2) -- (#1+#3+\cwsx,#2+\cwsy) -- (#1+\cwsx,#2+\cwsy) -- cycle;}
\newcommand{\cwflat}[6]{%
  \begin{scope}[shift={(#2,#3)},cm={1,0,\cwdx,\cwdy,(0,0)}]
    \node[inner sep=0pt,anchor=south west,transform shape] (#1) at (0,0) {\includegraphics[width=#4pt,height=#5pt]{figures/tikz/assets/cw/#6}};
    \draw[white,line width=0.8pt] (0,0) rectangle (#4,#5);
    \coordinate (#1-c) at (#4/2,#5/2); \coordinate (#1-fl) at (0,0); \coordinate (#1-fr) at (#4,0);
    \coordinate (#1-bl) at (0,#5); \coordinate (#1-br) at (#4,#5);
  \end{scope}}
\newcommand{\cwcube}[4]{%
  \colorlet{cwcubec}{#4}%
  \pgfmathsetmacro{\cwcx}{#3*0.5*\cwdx}\pgfmathsetmacro{\cwcy}{#3*0.5*\cwdy}%
  \path[fill=cwcubec!55!white,draw=cwcubec!55!black,line width=0.3pt] (#1,#2+#3) -- ++(\cwcx,\cwcy) -- ++(#3,0) -- ++(-\cwcx,-\cwcy) -- cycle;
  \path[fill=cwcubec!80!black,draw=cwcubec!55!black,line width=0.3pt] (#1+#3,#2) -- ++(\cwcx,\cwcy) -- ++(0,#3) -- ++(-\cwcx,-\cwcy) -- cycle;
  \path[fill=cwcubec,draw=cwcubec!55!black,line width=0.3pt] (#1,#2) rectangle ++(#3,#3);}
\newcommand{\cwbar}[6]{%
  \colorlet{cwbarc}{#6}%
  \pgfmathsetmacro{\cwbx}{#4*\cwdx}\pgfmathsetmacro{\cwby}{#4*\cwdy}%
  \path[fill=cwbarc!80!black,draw=cwbarc!50!black,line width=0.35pt] (#1+#3,#2) -- ++(\cwbx,\cwby) -- ++(0,#5) -- ++(-\cwbx,-\cwby) -- cycle;
  \path[fill=cwbarc!45!white,draw=cwbarc!50!black,line width=0.35pt] (#1,#2+#5) -- ++(\cwbx,\cwby) -- ++(#3,0) -- ++(-\cwbx,-\cwby) -- cycle;
  \path[fill=cwbarc,draw=cwbarc!50!black,line width=0.35pt] (#1,#2) rectangle ++(#3,#5);}
\tikzset{
  card/.style={inner sep=0pt,draw=white,line width=0.8pt,blur shadow={shadow blur steps=5,shadow xshift=1pt,shadow yshift=-1.2pt,shadow opacity=35}},
  beam/.style={fill=cwHi,opacity=0.42},
  glow/.style={draw=cwHiD,line width=1.1pt},
}
\newcommand{\cwring}[6]{%
  \pgfmathsetmacro{\cwra}{90-360*#4}\pgfmathsetmacro{\cwrb}{\cwra-360*#5}%
  \draw[cwGray!25,line width=#6] (#1,#2) circle[radius=#3];
  \draw[cwA,line width=#6,line cap=butt] (#1,#2) ++(90:#3) arc[start angle=90,end angle=\cwra,radius=#3];
  \draw[cwB,line width=#6,line cap=butt] (#1,#2) ++(\cwra:#3) arc[start angle=\cwra,end angle=\cwrb,radius=#3];
  \draw[white,line width=0.3pt] (#1,#2) circle[radius=#3+#6/2] (#1,#2) circle[radius=#3-#6/2];}
\newcommand{\cwspark}[3]{%
  \foreach \cwang in {0,45,...,315}{\draw[cwGold,line width=0.6pt] (#1,#2) ++(\cwang:#3*0.35) -- ++(\cwang:#3*0.65);}
  \fill[cwGold] (#1,#2) circle[radius=#3*0.18];}
\newcommand{\cwgauge}[5]{%
  \foreach \cwg in {1,...,#4}{%
    \pgfmathsetmacro{\cwga}{180-(\cwg-1)*180/#4-2}\pgfmathsetmacro{\cwgb}{180-\cwg*180/#4+2}%
    \ifnum\cwg>#5 \def\cwgc{cwHGrey}\else\def\cwgc{cwAd}\fi
    \draw[\cwgc,line width=4.2pt,line cap=butt] (#1,#2) ++(\cwga:#3) arc[start angle=\cwga,end angle=\cwgb,radius=#3];}
  \draw[cwInk,line width=0.7pt,-{Stealth[length=3pt]}] (#1,#2) -- ++({180-#5*180/#4}:#3-4);
  \fill[cwInk] (#1,#2) circle[radius=1.4pt];}
\tikzset{
  glowA/.style={draw=cwA,line width=4.2pt,opacity=0.22,line cap=round},
  glowB/.style={draw=cwB,line width=4.2pt,opacity=0.25,line cap=round},
  glowG/.style={draw=cwGold,line width=4.2pt,opacity=0.3,line cap=round},
  gold/.style={draw=cwGold,line width=1.2pt},
  poison/.style={left color=cwBad!8,right color=cwBad!45},
}
\definecolor{cwOurs}{HTML}{4F46A5}\definecolor{cwOursL}{HTML}{DEDCF3}\definecolor{cwOursM}{HTML}{A7A2DB}% CoWeave: indigo, the hue of Fig. 2 (4)
\newcommand{\cwpcard}[5]{%
  \path[fill=cwInk!3.5,rounded corners=4pt] (#1,#2) rectangle (#3,#4);
  \node[anchor=north west,inner sep=0pt,font=\footnotesize\bfseries,text=cwInk] at (#1+5,#4-4.5) {#5};}
\tikzset{sc/.style={inner sep=0pt,font=\fontsize{7.4}{8.4}\selectfont\scshape,text=cwNote}}
\pgfplotsset{/tikz/fill between/on layer=main}
\definecolor{cwB1}{HTML}{4F565F}\definecolor{cwB2}{HTML}{7E848C}\definecolor{cwB3}{HTML}{A2A7AE}\definecolor{cwB4}{HTML}{C3C7CC}\definecolor{cwL3}{HTML}{8A9098}\definecolor{cwL4}{HTML}{A6ABB2}% plot lines
\pgfplotsset{cw axis/.style={%
  scale only axis, axis lines=left, axis line style={cwInk!65,line width=0.5pt,-},%
  every tick/.style={cwInk!65,line width=0.45pt}, tick align=outside, major tick length=2pt,%
  tick label style={font=\footnotesize,text=cwInk}, label style={font=\footnotesize,text=cwInk},%
  xlabel style={yshift=2.6pt}, ylabel style={yshift=-3pt},%
  ymajorgrids, every axis grid/.style={}, grid style={cwInk!9,line width=0.45pt,-}, clip mode=individual}}
\input{figures/tikz/cw_boxes}


==> figures/tikz/cw_boxes.tex <==
\expandafter\def\csname cwbox@m_c03_1370-A\endcsname{0.1218/0.0536/0.3959/0.7739}%
\expandafter\def\csname cwbox@m_c03_1370-B\endcsname{0.6467/0.1597/0.8782/0.9464}%
\expandafter\def\csname cwbox@m_c08_1011-A\endcsname{0.2261/0.0207/0.3997/0.6919}%
\expandafter\def\csname cwbox@m_c08_1011-B\endcsname{0.3598/0.3260/0.4725/0.9136}%
\expandafter\def\csname cwbox@m_c12_5544-A\endcsname{0.3215/0.0199/0.5252/0.8770}%
\expandafter\def\csname cwbox@m_c12_5544-B\endcsname{0.4269/0.0040/0.6883/0.7499}%
\expandafter\def\csname cwbox@m_c03_1433-A\endcsname{0.3659/0.2538/0.5379/0.8225}%
\expandafter\def\csname cwbox@m_c03_1433-B\endcsname{0.5472/0.0040/0.7034/0.5468}%
\expandafter\def\csname cwbox@m_c08_1068-A\endcsname{0.3598/0.1726/0.6402/0.8145}%
\expandafter\def\csname cwbox@m_c08_1068-B\endcsname{0.4768/0.5128/0.5973/0.9960}%
\expandafter\def\csname cwbox@o_A_c04_92-C\endcsname{0.1875/-0.7534/0.8808/0.9363}%
\expandafter\def\csname cwbox@o_A_c04_92_ctx-C\endcsname{0.4544/0.2397/0.5556/0.6886}%
\expandafter\def\csname cwbox@o_A_c04_92_ctx-P\endcsname{0.4445/0.3087/0.5555/0.6913}%
\expandafter\def\csname cwbox@o_A_c04_345-C\endcsname{0.1429/-0.4999/0.8202/0.9700}%
\expandafter\def\csname cwbox@o_A_c04_345_ctx-C\endcsname{0.1002/0.4935/0.1905/0.8506}%
\expandafter\def\csname cwbox@o_A_c04_345_ctx-P\endcsname{0.1049/0.4950/0.1907/0.8449}%
\expandafter\def\csname cwbox@o_A_c02_345-C\endcsname{0.1593/-0.4834/0.8023/0.8970}%
\expandafter\def\csname cwbox@o_A_c02_345_ctx-C\endcsname{0.4568/0.3361/0.5383/0.6549}%
\expandafter\def\csname cwbox@o_A_c02_345_ctx-P\endcsname{0.4601/0.3337/0.5399/0.6663}%
\expandafter\def\csname cwbox@o_A_c02_368-C\endcsname{0.1447/-0.5160/0.8417/0.9030}%
\expandafter\def\csname cwbox@o_A_c02_368_ctx-C\endcsname{0.4521/0.3176/0.5461/0.6662}%
\expandafter\def\csname cwbox@o_A_c02_368_ctx-P\endcsname{0.4552/0.3231/0.5448/0.6769}%
\expandafter\def\csname cwbox@o_B_c02_575-C\endcsname{0.1131/0.0000/0.9791/0.5347}%
\expandafter\def\csname cwbox@o_B_c02_575_ctx-C\endcsname{0.4278/0.0000/0.5894/0.1818}%
\expandafter\def\csname cwbox@o_B_c02_575_ctx-P\endcsname{0.4167/0.0040/0.5833/0.1787}%
\expandafter\def\csname cwbox@o_B_c03_1380-M\endcsname{-0.2882/-0.1745/1.0835/1.0168}%
\expandafter\def\csname cwbox@o_B_c03_1380-C\endcsname{0.0495/-0.3088/0.9155/0.9269}%
\expandafter\def\csname cwbox@o_B_c03_1380_ctx-M\endcsname{0.1747/0.2826/0.4759/0.7591}%
\expandafter\def\csname cwbox@o_B_c03_1380_ctx-C\endcsname{0.2489/0.2289/0.4391/0.7232}%
\expandafter\def\csname cwbox@o_B_c03_1380_ctx-P\endcsname{0.2498/0.2265/0.4458/0.7231}%
\expandafter\def\csname cwbox@o_B_c03_1403-M\endcsname{-0.0054/-0.1653/0.9196/0.9651}%
\expandafter\def\csname cwbox@o_B_c03_1403-C\endcsname{0.1799/-0.4914/0.8237/0.9487}%
\expandafter\def\csname cwbox@o_B_c03_1403_ctx-M\endcsname{0.3614/0.4013/0.5655/0.8555}%
\expandafter\def\csname cwbox@o_B_c03_1403_ctx-C\endcsname{0.4023/0.2703/0.5443/0.8489}%
\expandafter\def\csname cwbox@o_B_c03_1403_ctx-P\endcsname{0.4041/0.2694/0.5417/0.8480}%
\expandafter\def\csname cwbox@o_B_c03_1449-M\endcsname{0.0275/-0.2586/0.8829/1.0713}%
\expandafter\def\csname cwbox@o_B_c03_1449-C\endcsname{0.1108/0.0479/0.7332/0.9472}%
\expandafter\def\csname cwbox@o_B_c03_1449_ctx-M\endcsname{0.4037/0.2921/0.5780/0.7858}%
\expandafter\def\csname cwbox@o_B_c03_1449_ctx-C\endcsname{0.4207/0.4059/0.5475/0.7397}%
\expandafter\def\csname cwbox@o_B_c03_1449_ctx-P\endcsname{0.4241/0.2049/0.5759/0.7394}%
\expandafter\def\csname cwbox@o_C_c05_1104-C\endcsname{0.1629/-0.4946/0.7914/0.9710}%
\expandafter\def\csname cwbox@o_C_c05_1104_ctx-C\endcsname{0.4616/0.3842/0.5332/0.6879}%
\expandafter\def\csname cwbox@o_C_c05_1104_ctx-P\endcsname{0.4696/0.3844/0.5304/0.6828}%
\expandafter\def\csname cwbox@o_C_c01_1127-C\endcsname{0.1419/-0.4560/0.8674/0.9484}%
\expandafter\def\csname cwbox@o_C_c01_1127_ctx-C\endcsname{0.4478/0.3187/0.5536/0.6918}%
\expandafter\def\csname cwbox@o_C_c01_1127_ctx-P\endcsname{0.4471/0.3087/0.5529/0.6913}%
\expandafter\def\csname cwbox@o_C_c01_1150-C\endcsname{0.1869/-0.4644/0.8131/0.9476}%
\expandafter\def\csname cwbox@o_C_c01_1150_ctx-C\endcsname{0.4543/0.3165/0.5457/0.6917}%
\expandafter\def\csname cwbox@o_C_c01_1150_ctx-P\endcsname{0.4516/0.3087/0.5484/0.6913}%
\expandafter\def\csname cwbox@o_C_c01_1449_ctx-P\endcsname{0.4742/0.4355/0.5257/0.6361}%
\expandafter\def\csname cwbox@o_D_c03_1127-M\endcsname{0.0040/0.2005/1.0624/1.0692}%
\expandafter\def\csname cwbox@o_D_c03_1127-C\endcsname{0.0576/0.2360/0.9476/0.9259}%
\expandafter\def\csname cwbox@o_D_c03_1127_ctx-M\endcsname{0.5368/0.1589/0.7822/0.5257}%
\expandafter\def\csname cwbox@o_D_c03_1127_ctx-C\endcsname{0.5492/0.1739/0.7556/0.4652}%
\expandafter\def\csname cwbox@o_D_c03_1127_ctx-P\endcsname{0.5483/0.0040/0.7553/0.4656}%
\expandafter\def\csname cwbox@o_D_c03_1150-M\endcsname{0.0687/0.1345/1.0843/1.0105}%
\expandafter\def\csname cwbox@o_D_c03_1150-C\endcsname{0.0831/0.0224/0.9508/0.9161}%
\expandafter\def\csname cwbox@o_D_c03_1150_ctx-M\endcsname{0.4979/0.0650/0.7673/0.4882}%
\expandafter\def\csname cwbox@o_D_c03_1150_ctx-C\endcsname{0.5017/0.0108/0.7318/0.4426}%
\expandafter\def\csname cwbox@o_D_c03_1150_ctx-P\endcsname{0.4939/0.0040/0.7307/0.4459}%
\expandafter\def\csname cwbox@o_D_c03_1173-M\endcsname{0.0024/0.0040/1.2475/0.8166}%
\expandafter\def\csname cwbox@o_D_c03_1173-C\endcsname{0.0386/0.0142/0.9655/0.7681}%
\expandafter\def\csname cwbox@o_D_c03_1173_ctx-M\endcsname{0.4412/0.0021/0.8007/0.4295}%
\expandafter\def\csname cwbox@o_D_c03_1173_ctx-C\endcsname{0.4516/0.0075/0.7193/0.4040}%
\expandafter\def\csname cwbox@o_D_c03_1173_ctx-P\endcsname{0.4559/0.0040/0.7138/0.4008}%
\expandafter\def\csname cwbox@o_D_c03_1196-M\endcsname{0.0559/0.0089/1.1881/0.6791}%
\expandafter\def\csname cwbox@o_D_c03_1196-C\endcsname{0.1004/0.0043/0.9603/0.6096}%
\expandafter\def\csname cwbox@o_D_c03_1196_ctx-M\endcsname{0.3998/0.0047/0.7316/0.3625}%
\expandafter\def\csname cwbox@o_D_c03_1196_ctx-C\endcsname{0.4128/0.0023/0.6648/0.3254}%
\expandafter\def\csname cwbox@o_D_c03_1196_ctx-P\endcsname{0.3991/0.0040/0.6608/0.3284}%


==> figures/tikz/supp_coweave_style.tex <==
\providecommand{\cwStyleLoaded}{}
\definecolor{cwA}{HTML}{5FB8C2}      % identity A, teal (fills, bars)
\definecolor{cwB}{HTML}{F2A0C8}      % identity B, rose (fills, bars)
\definecolor{cwC}{HTML}{B4A7D6}      % identity C
\definecolor{cwAd}{HTML}{1A7F8E}     % identity A, strokes and letters (4.6:1 on white)
\definecolor{cwBd}{HTML}{B8418A}     % identity B, strokes and letters (5.0:1 on white); magenta side, apart from the coral error red
\definecolor{cwCd}{HTML}{7A6AB5}
\definecolor{cwOK}{HTML}{548235}     % correct (glyphs)
\definecolor{cwBad}{HTML}{D36265}    % wrong (glyphs, the focal error line)
\definecolor{cwGray}{HTML}{6B6B6B}   % new / unresolved / unknown (strokes, text)
\definecolor{cwInk}{HTML}{222222}
\definecolor{cwNote}{HTML}{5A5A5A}   % secondary text (6.9:1 on white)
\definecolor{cwPanel}{HTML}{F1F3F4}  % the CoWeave band only
\definecolor{cwRule}{HTML}{8F999F}   % dividers (3.0:1 on white)
\definecolor{cwHair}{HTML}{C9CFD3}   % panel separators
\definecolor{cwYel}{HTML}{F0E442}    % annotated person in observed-output figures
\tikzset{
  cw/.style={x=1pt,y=1pt,line cap=round,line join=round,font=\scriptsize,text=cwInk},
  panel/.style={fill=none,draw=none},
  ptitle/.style={anchor=north west,inner sep=0pt,font=\footnotesize\bfseries},
  psub/.style={anchor=north west,inner sep=0pt,font=\scriptsize,text=cwNote},
  plab/.style={inner sep=0pt,font=\scriptsize},
  phead/.style={inner sep=0pt,font=\scriptsize\bfseries},
  pnote/.style={inner sep=0pt,font=\scriptsize\itshape,text=cwNote},
  idn/.style={circle,draw=#1d,line width=0.6pt,shading=radial,inner color=white,outer color=#1!42,minimum size=11.5pt,inner sep=0pt,font=\scriptsize\bfseries,text=#1d!80!black},
  obs/.style={circle,draw=cwInk!75,line width=0.5pt,fill=white,minimum size=11.5pt,inner sep=0pt,font=\scriptsize},
  out/.style={rounded corners=2.5pt,draw=#1d,line width=0.8pt,fill=#1!16,minimum height=10.5pt,minimum width=15pt,inner sep=1.5pt,font=\scriptsize\bfseries,text=#1d},
  newid/.style={rounded corners=2.5pt,draw=cwGray,line width=0.5pt,fill=white,minimum height=10.5pt,minimum width=15pt,inner sep=1.5pt,font=\scriptsize\itshape,text=cwGray},
  unres/.style={rounded corners=2.5pt,draw=cwGray,dash pattern=on 1.6pt off 1.2pt,line width=0.6pt,fill=white,minimum height=10.5pt,minimum width=15pt,inner sep=1.5pt,font=\scriptsize,text=cwGray},
  ctx/.style={draw=cwInk!70,line width=0.5pt,dash pattern=on 2pt off 1.5pt},
  link/.style={draw=cwInk!80,line width=0.8pt},
  cand/.style={draw=cwInk!55,line width=0.5pt},
  flow/.style={draw=cwInk,line width=0.8pt,-{Stealth[length=4pt,width=3.4pt]}},
  thin/.style={draw=cwInk,line width=0.5pt,-{Stealth[length=3pt,width=2.6pt]}},
  tag/.style={fill=white,draw=cwInk!70,line width=0.5pt,inner sep=1pt,font=\scriptsize\bfseries},
  photo/.style={inner sep=0pt,draw=cwInk!45,line width=0.5pt},
  okmark/.style={text=cwOK,font=\footnotesize\bfseries,inner sep=0pt},
  badmark/.style={text=cwBad,font=\footnotesize\bfseries,inner sep=0pt},
  oursband/.style={fill=cwPanel,draw=none},
  hair/.style={draw=cwHair,line width=0.5pt},
}
\newcommand{\cwok}{\ensuremath{\checkmark}}
\newcommand{\cwbad}{\ensuremath{\boldsymbol{\times}}}
\newcommand{\cwown}[6]{%
  \pgfmathsetmacro{\cwoa}{#3*#5}\pgfmathsetmacro{\cwob}{#3*#6}%
  \fill[cwA!80] (#1,#2) rectangle ++(\cwoa,#4);
  \fill[cwB!80] (#1+\cwoa,#2) rectangle ++(\cwob,#4);
  \fill[cwGray!25] (#1+\cwoa+\cwob,#2) rectangle (#1+#3,#2+#4);
  \draw[cwInk!60,line width=0.5pt] (#1,#2) rectangle ++(#3,#4);}
\newcommand{\cwphoto}[7]{\node[photo,anchor=#7] (#1) at (#2,#3) {\includegraphics[width=#4pt,height=#5pt]{figures/tikz/assets/cw/#6}};}
\newcommand{\cwgt}[3]{%
  \edef\cwtmp{\csname cwbox@#2\endcsname}%
  \expandafter\cwgtbody\cwtmp\relax{#1}{#3}}
\def\cwgtbody#1/#2/#3/#4\relax#5#6{%
  \path let \p1=(#5.south west), \p2=(#5.north east) in
    coordinate (cwgt-sw) at ({\x1+#1*(\x2-\x1)},{\y1+#2*(\y2-\y1)})
    coordinate (cwgt-ne) at ({\x1+#3*(\x2-\x1)},{\y1+#4*(\y2-\y1)});
  \draw[#6] (cwgt-sw) rectangle (cwgt-ne);}
\newcommand{\cwfeat}[5]{%
  \foreach \cwv [count=\cwi from 0] in {#5}{\fill[cwInk!\cwv] (#1+\cwi*#3,#2) rectangle ++(#3,#4);}
  \foreach \cwv [count=\cwi from 1] in {#5}{\xdef\cwn{\cwi}}%
  \draw[cwInk!60,line width=0.5pt] (#1,#2) rectangle ++(\cwn*#3,#4);}
\newcommand{\cwmat}[8]{%
  \fill[cwSup!#4] (#1,#2) rectangle ++(#3,#3);   \fill[cwSup!#5] (#1+#3,#2) rectangle ++(#3,#3);
  \fill[cwSup!#6] (#1,#2-#3) rectangle ++(#3,#3); \fill[cwSup!#7] (#1+#3,#2-#3) rectangle ++(#3,#3);
  \draw[cwInk!60,line width=0.5pt] (#1,#2-#3) rectangle ++(2*#3,2*#3) (#1+#3,#2-#3) -- ++(0,2*#3) (#1,#2) -- ++(2*#3,0);
  \ifnum#8>0
    \node[plab,anchor=south,font=\scriptsize\bfseries,text=cwAd] at (#1+0.5*#3,#2+#3+0.5) {A};
    \node[plab,anchor=south,font=\scriptsize\bfseries,text=cwBd] at (#1+1.5*#3,#2+#3+0.5) {B};\fi
  \ifnum#8=1
    \node[plab,anchor=east] at (#1-1,#2+0.5*#3) {$x$};
    \node[plab,anchor=east] at (#1-1,#2-0.5*#3) {$y$};
  \fi}
\tikzset{cam/.pic={
  \path[fill=cwInk!80,rounded corners=0.5pt] (-3.5,-1.6) rectangle (0.9,1.6);
  \path[fill=cwInk!80] (0.9,-0.4) -- (3.5,-1.7) -- (3.5,1.7) -- (0.9,0.4) -- cycle;}}
\newcommand{\cwfov}[6]{%
  \fill[cwInk!10] (#1,#2) -- ++(#3-28:#4) arc[start angle=#3-28,end angle=#3+28,radius=#4] -- cycle;
  \draw[cwInk!35,line width=0.5pt] (#1,#2) -- ++(#3-28:#4) (#1,#2) -- ++(#3+28:#4);
  \pic[rotate=#3] at (#1,#2) {cam};
  \node[plab,font=\scriptsize\bfseries,anchor=#6,outer sep=5pt] at (#1,#2) {#5};}
\newcommand{\cwcam}[2]{%
  \path[fill=cwInk!80,rounded corners=0.6pt] (#1,#2-2.2) rectangle ++(5.6,4.4);
  \path[fill=cwInk!80] (#1+5.6,#2-0.6) -- (#1+8.6,#2-2.2) -- (#1+8.6,#2+2.2) -- (#1+5.6,#2+0.6) -- cycle;}
\newcommand{\cwlock}[2]{%
  \draw[cwInk,line width=0.6pt] (#1-1.6,#2+1.2) -- (#1-1.6,#2+2.6) arc[start angle=180,end angle=0,radius=1.6pt] -- (#1+1.6,#2+1.2);
  \path[fill=white,draw=cwInk,line width=0.6pt,rounded corners=0.5pt] (#1-2.6,#2-2.4) rectangle (#1+2.6,#2+1.4);}
\newcommand{\cwenc}[6]{%
  \path[fill=cwInk!8,draw=cwInk!70,line width=0.6pt,rounded corners=1pt] (#2,#3-#5/2) -- (#2+#4,#3-#6/2) -- (#2+#4,#3+#6/2) -- (#2,#3+#5/2) -- cycle;
  \coordinate (#1-in) at (#2,#3); \coordinate (#1-out) at (#2+#4,#3);}
\definecolor{cwTAmber}{HTML}{FFF1CC} \definecolor{cwLAmber}{HTML}{E2B33C} \definecolor{cwHAmber}{HTML}{FFE699}
\definecolor{cwTGrey}{HTML}{F3F7F9}  \definecolor{cwLGrey}{HTML}{899FA5}  \definecolor{cwHGrey}{HTML}{C4D4DD}
\definecolor{cwTRose}{HTML}{FDF0F3}  \definecolor{cwLRose}{HTML}{D99AB3}  \definecolor{cwHRose}{HTML}{FBDCE0}
\definecolor{cwTGreen}{HTML}{E8F3E2} \definecolor{cwLGreen}{HTML}{8DBF6E}  \definecolor{cwHGreen}{HTML}{C7E4B3}
\definecolor{cwTBad}{HTML}{FDF0F3}   \definecolor{cwLBad}{HTML}{D36265}   \definecolor{cwHBad}{HTML}{FBDCE0}
\definecolor{cwTGood}{HTML}{E8F3E2}  \definecolor{cwLGood}{HTML}{8DBF6E}  \definecolor{cwHGood}{HTML}{C7E4B3}
\definecolor{cwHi}{HTML}{FFE699}     \definecolor{cwHiD}{HTML}{BF9000}    % key-claim highlight (yellow)
\definecolor{cwSup}{HTML}{8C8CE0}    \definecolor{cwSupL}{HTML}{CECEFA}   % support / score (lavender ramp)
\definecolor{cwTokA}{HTML}{99CCFF} \definecolor{cwTokB}{HTML}{C7E4B3} \definecolor{cwTokC}{HTML}{FFE699} \definecolor{cwTokD}{HTML}{CECEFA}
\definecolor{cwTSky}{HTML}{E4F6FC} \definecolor{cwLSky}{HTML}{9DC3E6} \definecolor{cwHSky}{HTML}{DDEAF7}
\definecolor{cwGold}{HTML}{FFC000} \definecolor{cwGoldL}{HTML}{FFF1C9} \definecolor{cwPeach}{HTML}{F8CAAC}
\definecolor{cwGlass}{HTML}{E4F6FC} \definecolor{cwGlassL}{HTML}{A8CFE8}
\definecolor{cwFeat}{HTML}{55636F}
\newcommand{\cwbadge}[1]{\tikz[baseline=-0.62ex]\node[circle,fill=cwInk,text=white,inner sep=0pt,minimum size=8.4pt,font=\scriptsize\bfseries] {#1};}
\newcommand{\cwbox}[7]{%
  \path[fill=cwT#5,draw=cwL#5,line width=0.75pt,dash pattern=on 2.6pt off 1.7pt,rounded corners=4pt] (#1,#2) rectangle (#3,#4);
  \node[anchor=west,inner sep=0pt,font=\footnotesize\bfseries\itshape,text=cwInk] at (#1+4,#4-7.2) {\cwbadge{#6}\,\,#7};}
\newcommand{\cwtab}[6]{%
  \path[fill=cwH#5,draw=cwL#5,line width=0.6pt,rounded corners=3pt] (#1,#2) rectangle (#3,#4);
  \node[align=center,inner sep=0pt,font=\scriptsize\bfseries,text=cwInk] at ({(#1+#3)/2},{(#2+#4)/2}) {#6};}
\newcommand{\cwplate}[5]{%
  \path[fill=cwL#5!70,rounded corners=1pt] (#1,#3-#4/2-1.6) -- (#2,#3-#4/2-1.6) -- (#2+7,#3+#4/2-1.6) -- (#1+7,#3+#4/2-1.6) -- cycle;
  \path[fill=cwH#5,draw=cwL#5,line width=0.5pt,rounded corners=1pt] (#1,#3-#4/2) -- (#2,#3-#4/2) -- (#2+7,#3+#4/2) -- (#1+7,#3+#4/2) -- cycle;}
\newcommand{\cwtok}[5]{%
  \foreach \cwi in {1,...,#3}{\foreach \cwj in {1,...,#4}{
    \pgfmathtruncatemacro{\cwlv}{mod(\cwi*37+\cwj*53,50)+12}
    \pgfmathtruncatemacro{\cwtk}{mod(\cwi+2*\cwj,4)}%
    \ifcase\cwtk\def\cwtc{cwTokA}\or\def\cwtc{cwTokB}\or\def\cwtc{cwTokC}\else\def\cwtc{cwTokD}\fi
    \path[fill=\cwtc,draw=cwInk!55,line width=0.35pt] (#1+\cwi*#5-#5,#2-\cwj*#5) rectangle ++(#5,#5);}}
  \draw[cwInk!70,line width=0.5pt] (#1,#2-#4*#5) rectangle (#1+#3*#5,#2);}
\newcommand{\cwfilm}[4]{%
  \path[fill=cwInk!88,rounded corners=1.5pt] (#1,#2) rectangle (#3,#4);
  \pgfmathsetmacro{\cwfn}{floor((#3-#1-4)/6)}
  \foreach \cwk in {0,...,\cwfn}{\path[fill=white] (#1+3+\cwk*6,#2+1.1) rectangle ++(2.6,1.9);
    \path[fill=white] (#1+3+\cwk*6,#4-3) rectangle ++(2.6,1.9);}}
\tikzset{pill/.style={fill=cwGoldL,draw=cwHiD,line width=0.5pt,rounded corners=3pt,inner xsep=3pt,inner ysep=1.6pt,font=\scriptsize\itshape}}
\def\cwdx{0.55}\def\cwdy{0.42}
\newcommand{\cwslab}[6]{%
  \colorlet{cwslabt}{#5}\colorlet{cwslabe}{#6}%
  \pgfmathsetmacro{\cwsx}{#4*\cwdx}\pgfmathsetmacro{\cwsy}{#4*\cwdy}%
  \path[fill=cwslabe!55,blur shadow={shadow blur steps=6,shadow xshift=1.2pt,shadow yshift=-1.6pt,shadow opacity=25}]
     (#1,#2-3) -- (#1+#3,#2-3) -- (#1+#3+\cwsx,#2+\cwsy-3) -- (#1+#3+\cwsx,#2+\cwsy) -- (#1+\cwsx,#2+\cwsy) -- (#1,#2) -- cycle;
  \path[fill=cwslabe!70] (#1,#2-3) rectangle (#1+#3,#2);
  \path[fill=cwslabe!45] (#1+#3,#2-3) -- (#1+#3+\cwsx,#2+\cwsy-3) -- (#1+#3+\cwsx,#2+\cwsy) -- (#1+#3,#2) -- cycle;
  \path[top color=cwslabt!55,bottom color=cwslabt,draw=cwslabe,line width=0.5pt]
     (#1,#2) -- (#1+#3,#2) -- (#1+#3+\cwsx,#2+\cwsy) -- (#1+\cwsx,#2+\cwsy) -- cycle;}
\newcommand{\cwflat}[6]{%
  \begin{scope}[shift={(#2,#3)},cm={1,0,\cwdx,\cwdy,(0,0)}]
    \node[inner sep=0pt,anchor=south west,transform shape] (#1) at (0,0) {\includegraphics[width=#4pt,height=#5pt]{figures/tikz/assets/cw/#6}};
    \draw[white,line width=0.8pt] (0,0) rectangle (#4,#5);
    \coordinate (#1-c) at (#4/2,#5/2); \coordinate (#1-fl) at (0,0); \coordinate (#1-fr) at (#4,0);
    \coordinate (#1-bl) at (0,#5); \coordinate (#1-br) at (#4,#5);
  \end{scope}}
\newcommand{\cwcube}[4]{%
  \colorlet{cwcubec}{#4}%
  \pgfmathsetmacro{\cwcx}{#3*0.5*\cwdx}\pgfmathsetmacro{\cwcy}{#3*0.5*\cwdy}%
  \path[fill=cwcubec!55!white,draw=cwcubec!55!black,line width=0.3pt] (#1,#2+#3) -- ++(\cwcx,\cwcy) -- ++(#3,0) -- ++(-\cwcx,-\cwcy) -- cycle;
  \path[fill=cwcubec!80!black,draw=cwcubec!55!black,line width=0.3pt] (#1+#3,#2) -- ++(\cwcx,\cwcy) -- ++(0,#3) -- ++(-\cwcx,-\cwcy) -- cycle;
  \path[fill=cwcubec,draw=cwcubec!55!black,line width=0.3pt] (#1,#2) rectangle ++(#3,#3);}
\newcommand{\cwbar}[6]{%
  \colorlet{cwbarc}{#6}%
  \pgfmathsetmacro{\cwbx}{#4*\cwdx}\pgfmathsetmacro{\cwby}{#4*\cwdy}%
  \path[fill=cwbarc!80!black,draw=cwbarc!50!black,line width=0.35pt] (#1+#3,#2) -- ++(\cwbx,\cwby) -- ++(0,#5) -- ++(-\cwbx,-\cwby) -- cycle;
  \path[fill=cwbarc!45!white,draw=cwbarc!50!black,line width=0.35pt] (#1,#2+#5) -- ++(\cwbx,\cwby) -- ++(#3,0) -- ++(-\cwbx,-\cwby) -- cycle;
  \path[fill=cwbarc,draw=cwbarc!50!black,line width=0.35pt] (#1,#2) rectangle ++(#3,#5);}
\tikzset{
  card/.style={inner sep=0pt,draw=white,line width=0.8pt,blur shadow={shadow blur steps=5,shadow xshift=1pt,shadow yshift=-1.2pt,shadow opacity=35}},
  beam/.style={fill=cwHi,opacity=0.42},
  glow/.style={draw=cwHiD,line width=1.1pt},
}
\newcommand{\cwring}[6]{%
  \pgfmathsetmacro{\cwra}{90-360*#4}\pgfmathsetmacro{\cwrb}{\cwra-360*#5}%
  \draw[cwGray!25,line width=#6] (#1,#2) circle[radius=#3];
  \draw[cwA,line width=#6,line cap=butt] (#1,#2) ++(90:#3) arc[start angle=90,end angle=\cwra,radius=#3];
  \draw[cwB,line width=#6,line cap=butt] (#1,#2) ++(\cwra:#3) arc[start angle=\cwra,end angle=\cwrb,radius=#3];
  \draw[white,line width=0.3pt] (#1,#2) circle[radius=#3+#6/2] (#1,#2) circle[radius=#3-#6/2];}
\newcommand{\cwspark}[3]{%
  \foreach \cwang in {0,45,...,315}{\draw[cwGold,line width=0.6pt] (#1,#2) ++(\cwang:#3*0.35) -- ++(\cwang:#3*0.65);}
  \fill[cwGold] (#1,#2) circle[radius=#3*0.18];}
\newcommand{\cwgauge}[5]{%
  \foreach \cwg in {1,...,#4}{%
    \pgfmathsetmacro{\cwga}{180-(\cwg-1)*180/#4-2}\pgfmathsetmacro{\cwgb}{180-\cwg*180/#4+2}%
    \ifnum\cwg>#5 \def\cwgc{cwHGrey}\else\def\cwgc{cwAd}\fi
    \draw[\cwgc,line width=4.2pt,line cap=butt] (#1,#2) ++(\cwga:#3) arc[start angle=\cwga,end angle=\cwgb,radius=#3];}
  \draw[cwInk,line width=0.7pt,-{Stealth[length=3pt]}] (#1,#2) -- ++({180-#5*180/#4}:#3-4);
  \fill[cwInk] (#1,#2) circle[radius=1.4pt];}
\tikzset{
  glowA/.style={draw=cwA,line width=4.2pt,opacity=0.22,line cap=round},
  glowB/.style={draw=cwB,line width=4.2pt,opacity=0.25,line cap=round},
  glowG/.style={draw=cwGold,line width=4.2pt,opacity=0.3,line cap=round},
  gold/.style={draw=cwGold,line width=1.2pt},
  poison/.style={left color=cwBad!8,right color=cwBad!45},
}
\definecolor{cwOurs}{HTML}{4F46A5}\definecolor{cwOursL}{HTML}{DEDCF3}\definecolor{cwOursM}{HTML}{A7A2DB}% CoWeave: indigo, the hue of Fig. 2 (4)
\newcommand{\cwpcard}[5]{%
  \path[fill=cwInk!3.5,rounded corners=4pt] (#1,#2) rectangle (#3,#4);
  \node[anchor=north west,inner sep=0pt,font=\footnotesize\bfseries,text=cwInk] at (#1+5,#4-4.5) {#5};}
\tikzset{sc/.style={inner sep=0pt,font=\fontsize{7.4}{8.4}\selectfont\scshape,text=cwNote}}
\pgfplotsset{/tikz/fill between/on layer=main}
\definecolor{cwB1}{HTML}{4F565F}\definecolor{cwB2}{HTML}{7E848C}\definecolor{cwB3}{HTML}{A2A7AE}\definecolor{cwB4}{HTML}{C3C7CC}\definecolor{cwL3}{HTML}{8A9098}\definecolor{cwL4}{HTML}{A6ABB2}% plot lines
\pgfplotsset{cw axis/.style={%
  scale only axis, axis lines=left, axis line style={cwInk!65,line width=0.5pt,-},%
  every tick/.style={cwInk!65,line width=0.45pt}, tick align=outside, major tick length=2pt,%
  tick label style={font=\footnotesize,text=cwInk}, label style={font=\footnotesize,text=cwInk},%
  xlabel style={yshift=2.6pt}, ylabel style={yshift=-3pt},%
  ymajorgrids, every axis grid/.style={}, grid style={cwInk!9,line width=0.45pt,-}, clip mode=individual}}
\input{figures/tikz/supp_cw_boxes}


==> figures/tikz/supp_cw_boxes.tex <==
\expandafter\def\csname cwbox@m_c03_1370-A\endcsname{0.1218/0.0536/0.3959/0.7739}%
\expandafter\def\csname cwbox@m_c03_1370-B\endcsname{0.6467/0.1597/0.8782/0.9464}%
\expandafter\def\csname cwbox@m_c08_1011-A\endcsname{0.2261/0.0207/0.3997/0.6919}%
\expandafter\def\csname cwbox@m_c08_1011-B\endcsname{0.3598/0.3260/0.4725/0.9136}%
\expandafter\def\csname cwbox@m_c12_5544-A\endcsname{0.3215/0.0199/0.5252/0.8770}%
\expandafter\def\csname cwbox@m_c12_5544-B\endcsname{0.4269/0.0040/0.6883/0.7499}%
\expandafter\def\csname cwbox@m_c03_1433-A\endcsname{0.3659/0.2538/0.5379/0.8225}%
\expandafter\def\csname cwbox@m_c03_1433-B\endcsname{0.5472/0.0040/0.7034/0.5468}%
\expandafter\def\csname cwbox@m_c08_1068-A\endcsname{0.3598/0.1726/0.6402/0.8145}%
\expandafter\def\csname cwbox@m_c08_1068-B\endcsname{0.4768/0.5128/0.5973/0.9960}%
\expandafter\def\csname cwbox@o_A_c04_92-C\endcsname{0.1875/-0.7534/0.8808/0.9363}%
\expandafter\def\csname cwbox@o_A_c04_92_ctx-C\endcsname{0.4544/0.2397/0.5556/0.6886}%
\expandafter\def\csname cwbox@o_A_c04_92_ctx-P\endcsname{0.4445/0.3087/0.5555/0.6913}%
\expandafter\def\csname cwbox@o_A_c04_345-C\endcsname{0.1429/-0.4999/0.8202/0.9700}%
\expandafter\def\csname cwbox@o_A_c04_345_ctx-C\endcsname{0.1002/0.4935/0.1905/0.8506}%
\expandafter\def\csname cwbox@o_A_c04_345_ctx-P\endcsname{0.1049/0.4950/0.1907/0.8449}%
\expandafter\def\csname cwbox@o_A_c02_345-C\endcsname{0.1593/-0.4834/0.8023/0.8970}%
\expandafter\def\csname cwbox@o_A_c02_345_ctx-C\endcsname{0.4568/0.3361/0.5383/0.6549}%
\expandafter\def\csname cwbox@o_A_c02_345_ctx-P\endcsname{0.4601/0.3337/0.5399/0.6663}%
\expandafter\def\csname cwbox@o_A_c02_368-C\endcsname{0.1447/-0.5160/0.8417/0.9030}%
\expandafter\def\csname cwbox@o_A_c02_368_ctx-C\endcsname{0.4521/0.3176/0.5461/0.6662}%
\expandafter\def\csname cwbox@o_A_c02_368_ctx-P\endcsname{0.4552/0.3231/0.5448/0.6769}%
\expandafter\def\csname cwbox@o_B_c02_575-C\endcsname{0.1131/0.0000/0.9791/0.5347}%
\expandafter\def\csname cwbox@o_B_c02_575_ctx-C\endcsname{0.4278/0.0000/0.5894/0.1818}%
\expandafter\def\csname cwbox@o_B_c02_575_ctx-P\endcsname{0.4167/0.0040/0.5833/0.1787}%
\expandafter\def\csname cwbox@o_B_c03_1380-M\endcsname{-0.2882/-0.1745/1.0835/1.0168}%
\expandafter\def\csname cwbox@o_B_c03_1380-C\endcsname{0.0495/-0.3088/0.9155/0.9269}%
\expandafter\def\csname cwbox@o_B_c03_1380_ctx-M\endcsname{0.1747/0.2826/0.4759/0.7591}%
\expandafter\def\csname cwbox@o_B_c03_1380_ctx-C\endcsname{0.2489/0.2289/0.4391/0.7232}%
\expandafter\def\csname cwbox@o_B_c03_1380_ctx-P\endcsname{0.2498/0.2265/0.4458/0.7231}%
\expandafter\def\csname cwbox@o_B_c03_1403-M\endcsname{-0.0054/-0.1653/0.9196/0.9651}%
\expandafter\def\csname cwbox@o_B_c03_1403-C\endcsname{0.1799/-0.4914/0.8237/0.9487}%
\expandafter\def\csname cwbox@o_B_c03_1403_ctx-M\endcsname{0.3614/0.4013/0.5655/0.8555}%
\expandafter\def\csname cwbox@o_B_c03_1403_ctx-C\endcsname{0.4023/0.2703/0.5443/0.8489}%
\expandafter\def\csname cwbox@o_B_c03_1403_ctx-P\endcsname{0.4041/0.2694/0.5417/0.8480}%
\expandafter\def\csname cwbox@o_B_c03_1449-M\endcsname{0.0275/-0.2586/0.8829/1.0713}%
\expandafter\def\csname cwbox@o_B_c03_1449-C\endcsname{0.1108/0.0479/0.7332/0.9472}%
\expandafter\def\csname cwbox@o_B_c03_1449_ctx-M\endcsname{0.4037/0.2921/0.5780/0.7858}%
\expandafter\def\csname cwbox@o_B_c03_1449_ctx-C\endcsname{0.4207/0.4059/0.5475/0.7397}%
\expandafter\def\csname cwbox@o_B_c03_1449_ctx-P\endcsname{0.4241/0.2049/0.5759/0.7394}%
\expandafter\def\csname cwbox@o_C_c05_1104-C\endcsname{0.1629/-0.4946/0.7914/0.9710}%
\expandafter\def\csname cwbox@o_C_c05_1104_ctx-C\endcsname{0.4616/0.3842/0.5332/0.6879}%
\expandafter\def\csname cwbox@o_C_c05_1104_ctx-P\endcsname{0.4696/0.3844/0.5304/0.6828}%
\expandafter\def\csname cwbox@o_C_c01_1127-C\endcsname{0.1419/-0.4560/0.8674/0.9484}%
\expandafter\def\csname cwbox@o_C_c01_1127_ctx-C\endcsname{0.4478/0.3187/0.5536/0.6918}%
\expandafter\def\csname cwbox@o_C_c01_1127_ctx-P\endcsname{0.4471/0.3087/0.5529/0.6913}%
\expandafter\def\csname cwbox@o_C_c01_1150-C\endcsname{0.1869/-0.4644/0.8131/0.9476}%
\expandafter\def\csname cwbox@o_C_c01_1150_ctx-C\endcsname{0.4543/0.3165/0.5457/0.6917}%
\expandafter\def\csname cwbox@o_C_c01_1150_ctx-P\endcsname{0.4516/0.3087/0.5484/0.6913}%
\expandafter\def\csname cwbox@o_C_c01_1449_ctx-P\endcsname{0.4742/0.4355/0.5257/0.6361}%
\expandafter\def\csname cwbox@o_D_c03_1127-M\endcsname{0.0040/0.2005/1.0624/1.0692}%
\expandafter\def\csname cwbox@o_D_c03_1127-C\endcsname{0.0576/0.2360/0.9476/0.9259}%
\expandafter\def\csname cwbox@o_D_c03_1127_ctx-M\endcsname{0.5368/0.1589/0.7822/0.5257}%
\expandafter\def\csname cwbox@o_D_c03_1127_ctx-C\endcsname{0.5492/0.1739/0.7556/0.4652}%
\expandafter\def\csname cwbox@o_D_c03_1127_ctx-P\endcsname{0.5483/0.0040/0.7553/0.4656}%
\expandafter\def\csname cwbox@o_D_c03_1150-M\endcsname{0.0687/0.1345/1.0843/1.0105}%
\expandafter\def\csname cwbox@o_D_c03_1150-C\endcsname{0.0831/0.0224/0.9508/0.9161}%
\expandafter\def\csname cwbox@o_D_c03_1150_ctx-M\endcsname{0.4979/0.0650/0.7673/0.4882}%
\expandafter\def\csname cwbox@o_D_c03_1150_ctx-C\endcsname{0.5017/0.0108/0.7318/0.4426}%
\expandafter\def\csname cwbox@o_D_c03_1150_ctx-P\endcsname{0.4939/0.0040/0.7307/0.4459}%
\expandafter\def\csname cwbox@o_D_c03_1173-M\endcsname{0.0024/0.0040/1.2475/0.8166}%
\expandafter\def\csname cwbox@o_D_c03_1173-C\endcsname{0.0386/0.0142/0.9655/0.7681}%
\expandafter\def\csname cwbox@o_D_c03_1173_ctx-M\endcsname{0.4412/0.0021/0.8007/0.4295}%
\expandafter\def\csname cwbox@o_D_c03_1173_ctx-C\endcsname{0.4516/0.0075/0.7193/0.4040}%
\expandafter\def\csname cwbox@o_D_c03_1173_ctx-P\endcsname{0.4559/0.0040/0.7138/0.4008}%
\expandafter\def\csname cwbox@o_D_c03_1196-M\endcsname{0.0559/0.0089/1.1881/0.6791}%
\expandafter\def\csname cwbox@o_D_c03_1196-C\endcsname{0.1004/0.0043/0.9603/0.6096}%
\expandafter\def\csname cwbox@o_D_c03_1196_ctx-M\endcsname{0.3998/0.0047/0.7316/0.3625}%
\expandafter\def\csname cwbox@o_D_c03_1196_ctx-C\endcsname{0.4128/0.0023/0.6648/0.3254}%
\expandafter\def\csname cwbox@o_D_c03_1196_ctx-P\endcsname{0.3991/0.0040/0.6608/0.3284}%


==> figures/tikz/sx_boxes.tex <==
\expandafter\def\csname sxbox@mtp_c03-A\endcsname{0.4531/0.2538/0.6014/0.8225}
\expandafter\def\csname sxbox@mtp_c08-A\endcsname{0.3054/0.3139/0.5059/0.8462}
\expandafter\def\csname sxbox@mtp_c12-A\endcsname{0.4835/0.0227/0.6733/0.8871}
\expandafter\def\csname sxh@wt-0-C1\endcsname{177}
\expandafter\def\csname sxh@wt-1-C1\endcsname{181}
\expandafter\def\csname sxh@wt-21-C1\endcsname{159}
\expandafter\def\csname sxbox@wtp_C1-0\endcsname{0.4885/0.7111/0.5135/0.8750}
\expandafter\def\csname sxbox@wtp_C1-1\endcsname{0.4813/0.7056/0.5062/0.8731}
\expandafter\def\csname sxbox@wtp_C1-21\endcsname{0.8599/0.7213/0.8875/0.8685}
\expandafter\def\csname sxh@wt-0-C2\endcsname{248}
\expandafter\def\csname sxh@wt-1-C2\endcsname{242}
\expandafter\def\csname sxh@wt-21-C2\endcsname{279}
\expandafter\def\csname sxbox@wtp_C2-0\endcsname{0.9005/0.7787/0.9417/1.0000}
\expandafter\def\csname sxbox@wtp_C2-1\endcsname{0.9021/0.7852/0.9417/1.0000}
\expandafter\def\csname sxbox@wtp_C2-21\endcsname{0.2880/0.7287/0.3349/0.9870}
\expandafter\def\csname sxh@wt-0-C3\endcsname{298}
\expandafter\def\csname sxh@wt-1-C3\endcsname{289}
\expandafter\def\csname sxh@wt-21-C3\endcsname{978}
\expandafter\def\csname sxbox@wtp_C3-0\endcsname{0.7917/0.5861/0.8396/0.8620}
\expandafter\def\csname sxbox@wtp_C3-1\endcsname{0.7646/0.5963/0.8099/0.8639}
\expandafter\def\csname sxbox@wtp_C3-21\endcsname{0.6880/0.0000/0.8479/0.5204}


==> figures/tikz/sx_gallery.tex <==
\newcommand{\sxgallery}[7]{%
\begin{tikzpicture}[cw,font=\footnotesize]
\pgfmathsetmacro{\gw}{#4}\pgfmathsetmacro{\gh}{#5}\def\gx{22}\def\gs{6}
\pgfmathsetmacro{\rowh}{\gh+20}
\foreach \scene/\first [count=\r from 0] in {#6}{
  \pgfmathsetmacro{\yt}{-\r*\rowh}
  \path[fill=cwTGrey,rounded corners=4pt] (\gx-4,\yt-\gh-12) rectangle (\gx+#3*\gw+#3*\gs-\gs+4,\yt+4);
  \cwtab{0}{\yt-\gh-12}{14}{\yt+4}{Grey}{\rotatebox{90}{\scriptsize \scene}}
  \foreach \v [count=\c from 0] in {#7}{
    \pgfmathtruncatemacro{\k}{\first+\c}
    \pgfmathsetmacro{\xl}{\gx+\c*(\gw+\gs)}
    \edef\gfile{#1_img\ifnum\k<10 0\fi\k.png}
    \sxcardg{\xl}{\yt}{\gw}{\gh}{\gfile}
    \node[anchor=north,inner sep=0pt,sc] at (\xl+\gw/2,\yt-\gh-3) {view \v};}}
\end{tikzpicture}}
\newcommand{\sxcardg}[5]{%
  \path[fill=black,opacity=0.17,rounded corners=3.4pt] (#1+1.6,#2-#4-1.6) rectangle (#1+#3+1.6,#2-1.2);
  \begin{scope}\clip[rounded corners=3pt] (#1,#2-#4) rectangle (#1+#3,#2);
    \node[inner sep=0pt,anchor=north west] at (#1,#2) {\includegraphics[width=#3pt,height=#4pt]{figures/tikz/assets/#5}};\end{scope}
  \path[draw=white,line width=0.9pt,rounded corners=3pt] (#1,#2-#4) rectangle (#1+#3,#2);}


==> figures/tikz/sx_style.tex <==
\providecommand{\sxStyleLoaded}{}
\definecolor{cwHAmberL}{HTML}{FFE699}\definecolor{cwLAmberL}{HTML}{BF9000}
\definecolor{cwHLav}{HTML}{DCD5F2}\definecolor{cwLLav}{HTML}{9B8ECF}\definecolor{cwTLav}{HTML}{F3F0FA}
\input{figures/tikz/sx_boxes}
\newcommand{\sxgt}[3]{%
  \edef\sxtmp{\csname sxbox@#2\endcsname}%
  \expandafter\sxgtbody\sxtmp\relax{#1}{#3}}
\def\sxgtbody#1/#2/#3/#4\relax#5#6{%
  \path let \p1=(#5.south west), \p2=(#5.north east) in
    coordinate (sxgt-sw) at ({\x1+#1*(\x2-\x1)},{\y1+#2*(\y2-\y1)})
    coordinate (sxgt-ne) at ({\x1+#3*(\x2-\x1)},{\y1+#4*(\y2-\y1)});
  \draw[#6] (sxgt-sw) rectangle (sxgt-ne);}
\newcommand{\sxtagbox}[5]{%
  \sxgt{#1}{#2}{white,line width=1.8pt,rounded corners=1pt}\sxgt{#1}{#2}{#3,line width=0.95pt,rounded corners=1pt}%
  \ifx n#5\node[fill=#3,text=white,inner sep=0.8pt,rounded corners=0.8pt,anchor=south west,font=\scriptsize\bfseries] at (sxgt-sw|-sxgt-ne) {#4};%
  \else\node[fill=#3,text=white,inner sep=0.8pt,rounded corners=0.8pt,anchor=south east,font=\scriptsize\bfseries] at (sxgt-ne) {#4};\fi}
\newcommand{\sxcard}[6]{%
  \path[fill=black,opacity=0.17,rounded corners=3.4pt] (#2+1.8,#3-#5-1.8) rectangle (#2+#4+1.8,#3-1.2);
  \begin{scope}\clip[rounded corners=3pt] (#2,#3-#5) rectangle (#2+#4,#3);
    \node[inner sep=0pt,anchor=north west] (#1) at (#2,#3) {\includegraphics[width=#4pt,height=#5pt]{figures/tikz/assets/sx/#6}};\end{scope}
  \path[draw=white,line width=0.9pt,rounded corners=3pt] (#2,#3-#5) rectangle (#2+#4,#3);}
\newcommand{\sxbead}[7]{%
  \path[fill=black,opacity=0.2,rounded corners=2pt] (#2-#4/2+1.2,#3-#5/2-1.3) rectangle (#2+#4/2+1.2,#3+#5/2-0.6);
  \begin{scope}\clip[rounded corners=2pt] (#2-#4/2,#3-#5/2) rectangle (#2+#4/2,#3+#5/2);
    \node[inner sep=0pt] (#1) at (#2,#3) {\includegraphics[width=#4pt,height=#5pt]{figures/tikz/assets/sx/#6}};\end{scope}
  \path[draw=white,line width=1.6pt,rounded corners=2pt] (#2-#4/2,#3-#5/2) rectangle (#2+#4/2,#3+#5/2);
  \path[draw=#7,line width=0.9pt,rounded corners=2pt] (#2-#4/2,#3-#5/2) rectangle (#2+#4/2,#3+#5/2);}
\newcommand{\sxbobbin}[3]{%
  \path[fill=#3,rounded corners=0.6pt] (#1-4,#2-5.2) rectangle (#1+4,#2+5.2);
  \foreach \dy in {-3.6,-1.8,0,1.8,3.6}{\draw[#3!55!white,line width=0.35pt] (#1-4,#2+\dy-0.5) -- (#1+4,#2+\dy+0.5);}
  \path[fill=cwInk!70,rounded corners=0.5pt] (#1-5.6,#2-6.8) rectangle (#1-4,#2+6.8) (#1+4,#2-6.8) rectangle (#1+5.6,#2+6.8);}
\newcommand{\sxknot}[3]{\fill[#3] (#1,#2) circle[radius=2.6]; \fill[white] (#1-0.7,#2+0.7) circle[radius=0.75];}
\newcommand{\sxcamhead}[4]{%
  \fill[cwInk!85] (#1-24,#2) circle[radius=5.6];
  \path[fill=white,rounded corners=0.4pt] (#1-27,#2-1.8) rectangle (#1-22.6,#2+1.8);
  \path[fill=white] (#1-22.6,#2-0.4) -- (#1-20.5,#2-1.8) -- (#1-20.5,#2+1.8) -- (#1-22.6,#2+0.4) -- cycle;
  \node[inner sep=0pt,anchor=west,font=\footnotesize\bfseries] at (#1-16,#2) {#3};
  \node[inner sep=0pt,anchor=west,sc] at (#1+2,#2-0.2) {#4};}
\tikzset{
  sxyarn/.style={draw=#1,line width=2.6pt,line cap=round,postaction={draw=#1!45!white,line width=1.1pt,line cap=round}},
  sxwarp/.style={draw=cwInk!22,line width=0.7pt},
  sxgap/.style={inner sep=1.2pt,fill=white,rounded corners=2pt,font=\scriptsize,text=cwNote},
  sxfr/.style={inner sep=0pt,font=\fontsize{6.4}{7}\selectfont,text=cwNote},
}


==> generated/supp_control_readings.tex <==
\newcommand{\RepairEver}{\pv{75}}
\newcommand{\RepairMedian}{\pv{5}}
\newcommand{\RepairHeld}{\pv{69}}
\newcommand{\RepairLost}{\pv{6}}
\newcommand{\RepairNever}{\pv{25}}
\newcommand{\RepairHeldPct}{\pv{92}}
\newcommand{\RetentionCo}{\pv{80.5}}
\newcommand{\RetentionBest}{\pv{72.7}}
\newcommand{\RetentionMargin}{\pv{7.8}}


==> generated/supp_numbers.tex <==
\newcommand{\GoalID}{\pv{80.5}}
\newcommand{\BaseID}{\pv{72.9}}
\newcommand{\DeltaID}{\pv{7.6}}
\newcommand{\GoalC}{\pv{86.5}}
\newcommand{\BaseC}{\pv{77.8}}
\newcommand{\GoalW}{\pv{2.5}}
\newcommand{\BaseW}{\pv{5.9}}
\newcommand{\IndepW}{\pv{9.0}}
\newcommand{\GoalN}{\pv{11.0}}
\newcommand{\BaseN}{\pv{16.3}}
\newcommand{\GoalP}{\pv{82.1}}
\newcommand{\BaseP}{\pv{67.0}}
\newcommand{\DeltaP}{\pv{15.1}}
\newcommand{\LeadZero}{\pv{8.7}}
\newcommand{\Wdelta}{\pv{3.4}}
\newcommand{\Wrelative}{\pv{57.6}}
\newcommand{\WrongMin}{\pv{5.9}}
\newcommand{\WrongMax}{\pv{8.3}}
\newcommand{\TimeDelta}{\pv{8.4}}
\newcommand{\GoalMs}{\pv{46.6}}
\newcommand{\BaseMs}{\pv{43.0}}
\newcommand{\MctrMs}{\pv{49.8}}
\newcommand{\InitShare}{\pv{7.9}}
\newcommand{\RetShare}{\pv{7.2}}
\newcommand{\InitPct}{\pv{52}}
\newcommand{\ReaderGain}{\pv{7.1}}
\newcommand{\MatcherGain}{\pv{7.3}}
\newcommand{\BothGain}{\pv{15.8}}
\newcommand{\InteractionP}{\pv{1.3}}
\newcommand{\InteractionPlo}{\pv{$-$1.6}}
\newcommand{\InteractionPhi}{\pv{4.2}}
\newcommand{\Interaction}{\pv{0.9}}
\newcommand{\InteractionLo}{\pv{$-$1.2}}
\newcommand{\InteractionHi}{\pv{2.9}}
\newcommand{\ReaderGainH}{\pv{3.2}}
\newcommand{\MatcherGainH}{\pv{3.6}}
\newcommand{\TransferMin}{\pv{4.6}}
\newcommand{\TransferMax}{\pv{7.4}}
\newcommand{\TransferPMin}{\pv{9.7}}
\newcommand{\TransferPMax}{\pv{15.6}}
\newcommand{\Arrivals}{\pv{10,783}}
\newcommand{\Complete}{\pv{8,647}}
\newcommand{\Episodes}{\pv{30}}
\newcommand{\BudgetShift}{\pv{3.9}}
\newcommand{\BudgetCap}{\pv{32}}
\newcommand{\CoScored}{\pv{7.2}}
\newcommand{\InScored}{\pv{3.3}}
\newcommand{\NativeCo}{\pv{82.1}}
\newcommand{\NativeGmt}{\pv{74.9}}
\newcommand{\NativeDelta}{\pv{7.2}}
\newcommand{\NativeDeltaP}{\pv{14.2}}
\newcommand{\AblFixedRet}{\pv{4.3}}
\newcommand{\AblInstance}{\pv{8.7}}
\newcommand{\AblFixedRetID}{\pv{1.3}}
\newcommand{\AblInstanceID}{\pv{6.1}}
\newcommand{\PermCost}{\pv{5.1}}
\newcommand{\ZeroCost}{\pv{5.1}}
\newcommand{\RetMarginID}{\pv{7.8}}
\newcommand{\RetBestID}{\pv{diverse}}
\newcommand{\RetMarginP}{\pv{11.7}}
\newcommand{\RetBestP}{\pv{task-aware independent}}
\newcommand{\SweepMinID}{\pv{77.0}}
\newcommand{\SweepMinP}{\pv{77.0}}
\newcommand{\RevGranoID}{\pv{78.6}}
\newcommand{\RevGranoW}{\pv{3.1}}
\newcommand{\RevGranoP}{\pv{78.4}}
\newcommand{\RevGran}{\pv{3.7}}
\newcommand{\RevGranID}{\pv{1.9}}
\newcommand{\SymArrivals}{\pv{431}}
\newcommand{\SymEpisodes}{\pv{7}}
\newcommand{\TransWcMin}{\pv{3.1}}
\newcommand{\TransWcMax}{\pv{4.0}}
\newcommand{\TransWgMin}{\pv{7.0}}
\newcommand{\TransWgMax}{\pv{7.8}}
\newcommand{\StoreSave}{\pv{6}}
\newcommand{\TransHMin}{\pv{4.9}}
\newcommand{\TransHMax}{\pv{6.8}}
\newcommand{\TransRcMin}{\pv{91.2}}
\newcommand{\TransRcMax}{\pv{93.2}}
\newcommand{\TransRgMin}{\pv{83.1}}
\newcommand{\TransRgMax}{\pv{85.1}}
\newcommand{\ReaderMs}{\pv{44.5}}
\newcommand{\TrackletMs}{\pv{45.2}}
\newcommand{\LeadReliable}{\pv{5.9}}
\newcommand{\LeadGroup}{\pv{19.4}}
\newcommand{\LeadSplit}{\pv{24.6}}
\newcommand{\LeadInvalid}{\pv{31.6}}
\newcommand{\QuarterCo}{\pv{74.2}}
\newcommand{\QuarterCoP}{\pv{71.4}}
\newcommand{\DoubleGmt}{\pv{74.2}}
\newcommand{\InvLossCo}{\pv{2.9}}
\newcommand{\InvLossGmt}{\pv{7.1}}
\newcommand{\SdMax}{\pv{0.8}}


==> generated/supp_rowmacros.tex <==
\def\RowsMainwide{%
Independent & \pv{68.8} & \pv{57.5} & \pv{68.4} & \pv{9.0} & \pv{22.6} & \pv{55.3} &  & \pv{40.2} & \pv{1.00} &  & \pv{65.0} & \pv{50.7} &  & \pv{61.9} & \pv{47.7} &  & \pv{58.5} & \pv{44.6} \\
DyGLIP & \pv{71.3} & \pv{59.0} & \pv{70.3} & \pv{8.3} & \pv{21.4} & \pv{58.6} &  & \pv{39.5} & \pv{0.99} &  & \pv{67.9} & \pv{54.3} &  & \pv{63.9} & \pv{51.6} &  & \pv{61.0} & \pv{47.2} \\
ReST & \pv{72.1} & \pv{60.9} & \pv{72.7} & \pv{7.6} & \pv{19.8} & \pv{62.2} &  & \pv{37.5} & \pv{0.88} &  & \pv{68.4} & \pv{59.1} &  & \pv{65.8} & \pv{55.4} &  & \pv{61.8} & \pv{51.6} \\
MCTR & \pv{72.7} & \tsecond{\pv{62.7}} & \pv{74.5} & \pv{6.5} & \pv{18.9} & \pv{64.2} &  & \pv{49.8} & \pv{0.71} &  & \pv{69.1} & \pv{58.9} &  & \pv{66.1} & \pv{56.2} &  & \pv{62.6} & \pv{54.6} \\
GMT (causal) & \tsecond{\pv{72.9}} & \pv{62.6} & \tsecond{\pv{77.8}} & \tsecond{\pv{5.9}} & \tsecond{\pv{16.3}} & \tsecond{\pv{67.0}} &  & \pv{43.0} & \pv{1.00} &  & \tsecond{\pv{70.2}} & \tsecond{\pv{63.5}} &  & \tsecond{\pv{66.6}} & \tsecond{\pv{59.9}} &  & \tsecond{\pv{63.1}} & \tsecond{\pv{56.0}} \\
\rowcolor{tabours}\textbf{CoWeave} & \tbest{\pv{80.5}} & \tbest{\pv{69.3}} & \tbest{\pv{86.5}} & \tbest{\pv{2.5}} & \tbest{\pv{11.0}} & \tbest{\pv{82.1}} &  & \pv{46.6} & \pv{0.94} &  & \tbest{\pv{74.8}} & \tbest{\pv{73.2}} &  & \tbest{\pv{74.0}} & \tbest{\pv{75.5}} &  & \tbest{\pv{69.3}} & \tbest{\pv{68.3}} \\
$\Delta$ & \dgood{\pv{$+$7.6}}\dci{\pv{1.1}} & \dgood{\pv{$+$6.7}} & \dgood{\pv{$+$8.7}}\dci{\pv{1.5}} & \dgood{\pv{$-$3.4}}\dci{\pv{0.3}} & \dgood{\pv{$-$5.3}} & \dgood{\pv{$+$15.1}}\dci{\pv{1.8}} &  & \tna & \tna &  & \dgood{\pv{$+$4.6}}\dci{\pv{1.1}} & \dgood{\pv{$+$9.7}} &  & \dgood{\pv{$+$7.4}}\dci{\pv{0.5}} & \dgood{\pv{$+$15.6}} &  & \dgood{\pv{$+$6.2}}\dci{\pv{1.5}} & \dgood{\pv{$+$12.3}} \\%
}
\def\RowsFrontend{%
Independent & \pv{70.1} & \pv{57.1} & \pv{1.00} \\
DyGLIP & \pv{73.1} & \pv{61.0} & \pv{1.17} \\
ReST & \pv{73.7} & \pv{64.3} & \pv{1.06} \\
MCTR & \pv{74.1} & \pv{66.2} & \pv{1.39} \\
GMT (causal) & \tsecond{\pv{74.9}} & \tsecond{\pv{69.8}} & \pv{1.26} \\
\rowcolor{tabours}\textbf{CoWeave} & \tbest{\pv{82.1}} & \tbest{\pv{84.0}} & \pv{1.34} \\
$\Delta$ & \dgood{\pv{$+$7.2}} & \dgood{\pv{$+$14.2}} &  \\%
}
\def\RowsAblationmain{%
\rowcolor{tabgroup}\multicolumn{5}{l}{\textit{\textbf{Single-part replacement, same read budget}}} \\
\rowcolor{tabours}\textbf{Full CoWeave} & \tbest{\pv{80.5}} & \tbest{\pv{2.5}} & \tbest{\pv{82.1}} & \tna \\
Fixed retrieval & \pv{79.2} & \pv{3.3} & \pv{77.8} & \dbad{\pv{$-$4.3}} \\
Zero relational support & \pv{77.1} & \pv{3.5} & \pv{77.0} & \dbad{\pv{$-$5.1}} \\
Tracklet-level reassignment & \pv{78.6} & \pv{3.1} & \pv{78.4} & \dbad{\pv{$-$3.7}} \\
Fixed record ownership & \pv{76.5} & \pv{3.8} & \pv{74.9} & \dbad{\pv{$-$7.2}} \\
Without instance detail & \pv{74.4} & \pv{4.5} & \pv{73.4} & \dbad{\pv{$-$8.7}} \\
\rowcolor{tabgroup}\multicolumn{5}{l}{\textit{\textbf{Retention policy, same storage cap}}} \\
\rowcolor{tabours}\textbf{Full CoWeave} & \tbest{\pv{80.5}} & \tbest{\pv{2.5}} & \tbest{\pv{82.1}} & \tna \\
Recent & \pv{72.1} & \pv{6.9} & \pv{65.8} & \dbad{\pv{$-$16.3}} \\
Diverse & \pv{72.7} & \pv{6.5} & \pv{68.4} & \dbad{\pv{$-$13.7}} \\
Task-aware independent & \pv{72.1} & \pv{5.8} & \pv{70.4} & \dbad{\pv{$-$11.7}} \\%
}
\def\StyIdcounts{%
Independent & \pv{896,394} & \pv{424,703} & \pv{388,762} & \pv{67.9} & \pv{69.8} & \pv{68.8} \\
DyGLIP & \pv{934,865} & \pv{403,387} & \pv{350,291} & \pv{69.9} & \pv{72.7} & \pv{71.3} \\
ReST & \pv{919,019} & \tsecond{\pv{346,670}} & \pv{366,137} & \tsecond{\pv{72.6}} & \pv{71.5} & \pv{72.1} \\
MCTR & \pv{940,455} & \pv{362,296} & \pv{344,700} & \pv{72.2} & \tsecond{\pv{73.2}} & \pv{72.7} \\
GMT (causal) & \tsecond{\pv{941,320}} & \pv{355,372} & \tsecond{\pv{343,836}} & \tsecond{\pv{72.6}} & \tsecond{\pv{73.2}} & \tsecond{\pv{72.9}} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{1,030,925}} & \tbest{\pv{245,567}} & \tbest{\pv{254,230}} & \tbest{\pv{80.8}} & \tbest{\pv{80.2}} & \tbest{\pv{80.5}} \\
$\Delta$ & \dgood{\pv{$+$89,605}} & \dgood{\pv{$-$109,805}} & \dgood{\pv{$-$89,606}} & \dgood{\pv{$+$8.2}} & \dgood{\pv{$+$7.0}} & \dgood{\pv{$+$7.6}} \\%
}
\def\StySeeds{%
Independent & \pv{68.8}\dci{\pv{0.13}} & \pv{57.5}\dci{\pv{0.25}} & \pv{68.4}\dci{\pv{0.33}} & \pv{9.0}\dci{\pv{0.18}} & \pv{22.6}\dci{\pv{0.48}} & \pv{55.3}\dci{\pv{0.33}} & \pv{80.9}\dci{\pv{0.32}} \\
DyGLIP & \pv{71.3}\dci{\pv{0.76}} & \pv{59.0}\dci{\pv{0.55}} & \pv{70.3}\dci{\pv{0.25}} & \pv{8.3}\dci{\pv{0.01}} & \pv{21.4}\dci{\pv{0.26}} & \pv{58.6}\dci{\pv{0.19}} & \pv{83.3}\dci{\pv{0.30}} \\
ReST & \pv{72.1}\dci{\pv{0.62}} & \pv{60.9}\dci{\pv{0.20}} & \pv{72.7}\dci{\pv{0.21}} & \pv{7.6}\dci{\pv{0.01}} & \pv{19.8}\dci{\pv{0.22}} & \pv{62.2}\dci{\pv{0.50}} & \pv{85.6}\dci{\pv{0.82}} \\
MCTR & \pv{72.7}\dci{\pv{0.53}} & \pv{62.7}\dci{\pv{0.62}} & \pv{74.5}\dci{\pv{0.49}} & \pv{6.5}\dci{\pv{0.10}} & \pv{18.9}\dci{\pv{0.50}} & \pv{64.2}\dci{\pv{0.46}} & \pv{86.1}\dci{\pv{1.18}} \\
GMT (causal) & \pv{72.9}\dci{\pv{0.06}} & \pv{62.6}\dci{\pv{0.22}} & \pv{77.8}\dci{\pv{0.45}} & \pv{5.9}\dci{\pv{0.12}} & \pv{16.3}\dci{\pv{0.56}} & \pv{67.0}\dci{\pv{0.58}} & \pv{86.2}\dci{\pv{0.28}} \\
\textbf{CoWeave} (ours) & \pv{80.5}\dci{\pv{0.50}} & \pv{69.3}\dci{\pv{0.27}} & \pv{86.5}\dci{\pv{0.48}} & \pv{2.5}\dci{\pv{0.10}} & \pv{11.0}\dci{\pv{0.54}} & \pv{82.1}\dci{\pv{0.45}} & \pv{94.9}\dci{\pv{0.31}} \\%
}
\def\StyPersistent{%
Independent & \pv{68.4} & \pv{65.5} & \pv{62.7} & \pv{58.4} & \pv{55.3} & \pv{80.9} \\
DyGLIP & \pv{70.3} & \pv{67.8} & \pv{65.3} & \pv{61.4} & \pv{58.6} & \pv{83.3} \\
ReST & \pv{72.7} & \pv{70.4} & \pv{68.2} & \pv{64.7} & \pv{62.2} & \pv{85.6} \\
MCTR & \pv{74.5} & \pv{72.2} & \pv{70.1} & \pv{66.7} & \pv{64.2} & \pv{86.1} \\
GMT (causal) & \tsecond{\pv{77.8}} & \tsecond{\pv{75.4}} & \tsecond{\pv{73.2}} & \tsecond{\pv{69.6}} & \tsecond{\pv{67.0}} & \tsecond{\pv{86.2}} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{86.5}} & \tbest{\pv{85.5}} & \tbest{\pv{84.6}} & \tbest{\pv{83.1}} & \tbest{\pv{82.1}} & \tbest{\pv{94.9}} \\
$\Delta$ & \dgood{\pv{$+$8.7}} & \dgood{\pv{$+$10.1}} & \dgood{\pv{$+$11.4}} & \dgood{\pv{$+$13.5}} & \dgood{\pv{$+$15.1}} & \dgood{\pv{$+$8.7}} \\%
}
\def\StyStored{%
Independent & \pv{1.00} & \pv{1.00} & \pv{40.2}\dci{\pv{0.31}} & \pv{58.9}\dci{\pv{1.35}} & \pv{1.00} \\
DyGLIP & \pv{0.98} & \pv{1.00} & \pv{39.5}\dci{\pv{1.01}} & \pv{58.6}\dci{\pv{1.69}} & \pv{0.99} \\
ReST & \pv{0.93} & \pv{0.94} & \pv{37.5}\dci{\pv{0.62}} & \pv{55.5}\dci{\pv{0.57}} & \pv{0.88} \\
MCTR & \pv{1.24} & \pv{1.25} & \pv{49.8}\dci{\pv{1.01}} & \pv{73.4}\dci{\pv{1.11}} & \pv{0.71} \\
GMT (causal) & \pv{1.07} & \pv{1.08} & \pv{43.0}\dci{\pv{0.28}} & \pv{63.3}\dci{\pv{1.32}} & \pv{1.00} \\
\textbf{CoWeave} (ours) & \pv{1.16} & \pv{1.17} & \pv{46.6}\dci{\pv{1.04}} & \pv{68.7}\dci{\pv{2.45}} & \pv{0.94} \\%
}
\def\StyCost{%
Independent & \pv{28.73} & \pv{3.27} & \pv{32} & \pv{40.2} & \pv{68.8} \\
GMT (causal) & \pv{27.64} & \pv{4.36} & \pv{32} & \pv{43.0} & \tsecond{\pv{72.9}} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \pv{24.82} & \pv{7.18} & \pv{32} & \pv{46.6} & \tbest{\pv{80.5}} \\%
}
\def\StyCrossed{%
Tracklet reader & GMT adapter & \pv{61.4} & \pv{72.1} & \pv{68.7} & \pv{66.3} & \pv{86.6} & \pv{45.2} & \pv{0.96} \\
Tracklet reader & CoWeave matcher & \tsecond{\pv{65.0}} & \pv{77.4} & \pv{75.2} & \tsecond{\pv{73.6}} & \tsecond{\pv{91.8}} & \pv{44.6} & \pv{0.96} \\
CoWeave reader & GMT adapter & \pv{64.6} & \tsecond{\pv{78.1}} & \tsecond{\pv{75.4}} & \pv{73.4} & \pv{89.9} & \pv{44.5} & \pv{0.96} \\
\rowcolor{tabours}CoWeave reader & CoWeave matcher & \tbest{\pv{69.3}} & \tbest{\pv{84.6}} & \tbest{\pv{83.1}} & \tbest{\pv{82.1}} & \tbest{\pv{94.9}} & \pv{46.6} & \pv{0.94} \\
$\Delta$ &  & \dgood{\pv{$+$7.9}} & \dgood{\pv{$+$12.5}} & \dgood{\pv{$+$14.4}} & \dgood{\pv{$+$15.8}} & \dgood{\pv{$+$8.3}} &  &  \\%
}
\def\StyBudget{%
0.25 & \pv{63.1} & \pv{65.1} & \tbest{\pv{74.2}} & \dgood{\pv{$+$9.1}} & \pv{71.4} \\
0.50 & \pv{66.5} & \pv{69.3} & \tbest{\pv{77.4}} & \dgood{\pv{$+$8.1}} & \pv{77.0} \\
1.00\,{\scriptsize\color{cwNote}default} & \pv{68.8} & \pv{72.9} & \tbest{\pv{80.5}} & \dgood{\pv{$+$7.6}} & \pv{82.1} \\
2.00 & \pv{70.0} & \pv{74.2} & \tbest{\pv{81.4}} & \dgood{\pv{$+$7.2}} & \pv{83.2} \\%
}
\def\StyValidity{%
0\%\,{\scriptsize\color{cwNote}default} & \pv{68.8} & \pv{72.9} & \tbest{\pv{80.5}} & \dgood{\pv{$+$7.6}} \\
10\% & \pv{68.8} & \pv{71.4} & \tbest{\pv{80.0}} & \dgood{\pv{$+$8.6}} \\
20\% & \pv{68.8} & \pv{69.4} & \tbest{\pv{79.4}} & \dgood{\pv{$+$10.0}} \\
30\% & \pv{68.8} & \pv{67.6} & \tbest{\pv{78.6}} & \dgood{\pv{$+$11.0}} \\
40\% & \pv{68.8} & \pv{65.8} & \tbest{\pv{77.6}} & \dgood{\pv{$+$11.8}} \\%
}
\def\StyDiagnostics{%
\rowcolor{tabgroup}\multicolumn{4}{l}{\textit{\textbf{Reliable relations and clear instance detail}}} \\
GMT (causal) & \pv{89.7} & \pv{3.2} & \pv{7.1} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{95.6}} & \tbest{\pv{1.2}} & \tbest{\pv{3.2}} \\
$\Delta$ & \dgood{\pv{$+$5.9}} & \dgood{\pv{$-$2.0}} & \dgood{\pv{$-$3.9}} \\
\rowcolor{tabgroup}\multicolumn{4}{l}{\textit{\textbf{Shared group and weak instance detail}}} \\
GMT (causal) & \pv{65.4} & \pv{12.3} & \pv{22.3} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{84.8}} & \tbest{\pv{3.3}} & \tbest{\pv{11.9}} \\
$\Delta$ & \dgood{\pv{$+$19.4}} & \dgood{\pv{$-$9.0}} & \dgood{\pv{$-$10.4}} \\
\rowcolor{tabgroup}\multicolumn{4}{l}{\textit{\textbf{Reappearance after group separation}}} \\
GMT (causal) & \pv{59.5} & \pv{15.4} & \pv{25.1} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{84.1}} & \tbest{\pv{3.6}} & \tbest{\pv{12.3}} \\
$\Delta$ & \dgood{\pv{$+$24.6}} & \dgood{\pv{$-$11.8}} & \dgood{\pv{$-$12.8}} \\
\rowcolor{tabgroup}\multicolumn{4}{l}{\textit{\textbf{Invalid relations and valid instance evidence}}} \\
GMT (causal) & \pv{51.6} & \pv{21.3} & \pv{27.1} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{83.2}} & \tbest{\pv{3.9}} & \tbest{\pv{12.9}} \\
$\Delta$ & \dgood{\pv{$+$31.6}} & \dgood{\pv{$-$17.4}} & \dgood{\pv{$-$14.2}} \\
\rowcolor{tabgroup}\multicolumn{4}{l}{\textit{\textbf{Complete symmetry (431 arrivals)}}} \\
GMT (causal) & \pv{0.0} & \pv{0.0} & \pv{100.0} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \pv{0.0} & \pv{0.0} & \pv{100.0} \\
$\Delta$ & \dzero{\pv{0.0}} & \dzero{\pv{0.0}} & \dzero{\pv{0.0}} \\%
}
\def\StyAblation{%
\rowcolor{tabours}\textbf{Full CoWeave} & \tbest{\pv{80.5}} & \tbest{\pv{86.5}} & \tbest{\pv{2.5}} & \tbest{\pv{11.0}} & \tbest{\pv{82.1}} \\
Fixed retrieval & \tsecond{\pv{79.2}} & \tsecond{\pv{84.5}} & \tsecond{\pv{3.3}} & \tsecond{\pv{12.2}} & \tsecond{\pv{77.8}} \\
Zero relational support & \pv{77.1} & \pv{83.7} & \pv{3.5} & \pv{12.8} & \pv{77.0} \\
Fixed record ownership & \pv{76.5} & \pv{82.0} & \pv{3.8} & \pv{14.2} & \pv{74.9} \\
Without instance detail & \pv{74.4} & \pv{81.4} & \pv{4.5} & \pv{14.1} & \pv{73.4} \\%
}
\def\StyRetention{%
Recent & \pv{72.1} & \pv{74.2} & \pv{6.9} & \pv{18.9} & \pv{65.8} \\
Diverse & \tsecond{\pv{72.7}} & \pv{75.9} & \pv{6.5} & \tsecond{\pv{17.5}} & \pv{68.4} \\
Task-aware independent & \pv{72.1} & \tsecond{\pv{76.5}} & \tsecond{\pv{5.8}} & \pv{17.7} & \tsecond{\pv{70.4}} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{80.5}} & \tbest{\pv{86.5}} & \tbest{\pv{2.5}} & \tbest{\pv{11.0}} & \tbest{\pv{82.1}} \\%
}
\def\StyIntervention{%
\rowcolor{tabours}\textbf{Original valid relations} & \tbest{\pv{69.3}} & \tbest{\pv{84.6}} & \tbest{\pv{83.1}} & \tbest{\pv{82.1}} & \tbest{\pv{94.9}} \\
No-operation control & \tbest{\pv{69.3}} & \tbest{\pv{84.6}} & \tbest{\pv{83.1}} & \tbest{\pv{82.1}} & \tbest{\pv{94.9}} \\
Degree-matched relation permutation & \tsecond{\pv{67.1}} & \tsecond{\pv{80.8}} & \tsecond{\pv{78.6}} & \tsecond{\pv{77.0}} & \tsecond{\pv{92.1}} \\
Zero relational support & \pv{66.1} & \tsecond{\pv{80.8}} & \tsecond{\pv{78.6}} & \tsecond{\pv{77.0}} & \pv{91.9} \\%
}
\def\StyCoverage{%
Independent & \pv{89.9} & \pv{83.8} & \pv{68.8} \\
GMT (causal) & \tsecond{\pv{92.0}} & \tsecond{\pv{86.9}} & \tsecond{\pv{72.9}} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{96.9}} & \tbest{\pv{95.1}} & \tbest{\pv{80.5}} \\
$\Delta$ & \dgood{\pv{$+$4.9}} & \dgood{\pv{$+$8.2}} & \dgood{\pv{$+$7.6}} \\%
}
\def\StyRepair{%
\rowcolor{tabgroup}\multicolumn{5}{l}{\textit{\textbf{(a) 100 events that start from an erroneous ownership snapshot}}} \\
Frozen ownership & \tsecond{\pv{0}} & \tsecond{\pv{78}} & \tsecond{\pv{22}} & \tna \\
Frozen, no-operation replay & \tsecond{\pv{0}} & \tsecond{\pv{78}} & \tsecond{\pv{22}} & \tna \\
\rowcolor{tabours}\textbf{Revisable ownership} & \tbest{\pv{69}} & \tbest{\pv{15}} & \tbest{\pv{16}} & \tna \\
$\Delta$ & \dgood{\pv{$+$69}} & \dgood{\pv{$-$63}} & \dgood{\pv{$-$6}} &  \\
\rowcolor{tabgroup}\multicolumn{5}{l}{\textit{\textbf{(b) 200 events that start from correct ownership}}} \\
Frozen ownership & \tbest{\pv{190}} & \tbest{\pv{4}} & \pv{6} & \tbest{\pv{0}} \\
\rowcolor{tabours}\textbf{Revisable ownership} & \pv{188} & \pv{6} & \pv{6} & \pv{2} \\
$\Delta$ & \dbad{\pv{$-$2}} & \dbad{\pv{$+$2}} & \dzero{\pv{0}} & \dbad{\pv{$+$2}} \\%
}
\def\StyTraining{%
0 & \pv{0.6918}\dci{\pv{0.003}} & \pv{0.9977}\dci{\pv{0.003}} & \pv{69.1}\dci{\pv{0.07}} \\
25 & \pv{0.3833}\dci{\pv{0.001}} & \pv{0.6139}\dci{\pv{0.004}} & \pv{75.2}\dci{\pv{0.17}} \\
50 & \pv{0.2455}\dci{\pv{0.002}} & \pv{0.3581}\dci{\pv{0.003}} & \pv{78.5}\dci{\pv{0.06}} \\
75 & \pv{0.1853}\dci{\pv{0.003}} & \pv{0.2783}\dci{\pv{0.002}} & \pv{80.2}\dci{\pv{0.17}} \\
100 & \pv{0.1681}\dci{\pv{0.002}} & \pv{0.2481}\dci{\pv{0.003}} & \pv{80.7}\dci{\pv{0.13}} \\%
}
\def\StyBootstrap{%
\rowcolor{tabgroup}\multicolumn{4}{l}{\textit{\textbf{CoWeave $-$ GMT (causal) on MTMMC}}} \\
G-IDF1 & \dgood{\pv{$+$7.57}} & \pv{[$+$6.57, $+$8.68]} & $\checkmark$ \\
Correct & \dgood{\pv{$+$8.67}} & \pv{[$+$7.19, $+$10.15]} & $\checkmark$ \\
Wrong & \dgood{\pv{$-$3.41}} & \pv{[$-$3.73, $-$3.09]} & $\checkmark$ \\
$P_{30}$ & \dgood{\pv{$+$15.04}} & \pv{[$+$13.23, $+$16.77]} & $\checkmark$ \\
\rowcolor{tabgroup}\multicolumn{4}{l}{\textit{\textbf{CoWeave $-$ GMT (causal) on other datasets}}} \\
WILDTRACK G-IDF1 & \dgood{\pv{$+$4.60}} & \pv{[$+$3.46, $+$5.74]} & $\checkmark$ \\
MMPTrack G-IDF1 & \dgood{\pv{$+$7.40}} & \pv{[$+$6.90, $+$7.90]} & $\checkmark$ \\
DIVOTrack G-IDF1 & \dgood{\pv{$+$6.20}} & \pv{[$+$4.71, $+$7.69]} & $\checkmark$ \\
\rowcolor{tabgroup}\multicolumn{4}{l}{\textit{\textbf{Reader $\times$ matcher interaction on MTMMC}}} \\
G-IDF1 & \pv{$+$0.88} & \pv{[$-$1.21, $+$2.89]} & \textcolor{cwNote}{no} \\
$P_{30}$ & \pv{$+$1.34} & \pv{[$-$1.62, $+$4.20]} & \textcolor{cwNote}{no} \\%
}
\def\StyReference{%
\rowcolor{tabgroup}\multicolumn{3}{l}{\textit{\textbf{Same causal RGB stream}}} \\
GMT (causal) & {\color{cwNote}Same RGB observations} & \pv{72.9} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & {\color{cwNote}Same RGB observations} & \tbest{\pv{80.5}} \\
\rowcolor{tabgroup}\multicolumn{3}{l}{\textit{\textbf{Additional information}}} \\
OCMCTrack & {\color{cwNote}Additional geometry} & \pv{76.0} \\
Lifted multicut & {\color{cwNote}Future tracklets} & \tsecond{\pv{78.7}} \\%
}
\def\StyTransfer{%
\rowcolor{tabgroup}\multicolumn{9}{l}{\textit{\textbf{WILDTRACK}}} \\
Independent & \pv{65.0} & \pv{54.9} & \pv{64.8} & \pv{9.6} & \pv{25.6} & \pv{50.7} & \pv{78.3} & \pv{40.8} \\
DyGLIP & \pv{67.9} & \pv{56.6} & \pv{65.5} & \pv{8.8} & \pv{25.8} & \pv{54.3} & \pv{82.9} & \pv{39.3} \\
ReST & \pv{68.4} & \pv{58.2} & \pv{68.8} & \pv{8.1} & \pv{23.1} & \pv{59.1} & \tsecond{\pv{85.9}} & \pv{37.8} \\
MCTR & \pv{69.1} & \pv{59.7} & \pv{70.9} & \pv{7.2} & \pv{21.9} & \pv{58.9} & \pv{83.1} & \pv{50.2} \\
GMT (causal) & \tsecond{\pv{70.2}} & \tsecond{\pv{60.3}} & \tsecond{\pv{74.6}} & \tsecond{\pv{7.0}} & \tsecond{\pv{18.4}} & \tsecond{\pv{63.5}} & \pv{85.1} & \pv{42.8} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{74.8}} & \tbest{\pv{65.2}} & \tbest{\pv{80.2}} & \tbest{\pv{3.4}} & \tbest{\pv{16.4}} & \tbest{\pv{73.2}} & \tbest{\pv{91.2}} & \pv{47.1} \\
$\Delta$ & \dgood{\pv{$+$4.6}} & \dgood{\pv{$+$4.9}} & \dgood{\pv{$+$5.6}} & \dgood{\pv{$-$3.6}} & \dgood{\pv{$-$2.0}} & \dgood{\pv{$+$9.7}} & \dgood{\pv{$+$6.1}} &  \\
\rowcolor{tabgroup}\multicolumn{9}{l}{\textit{\textbf{MMPTrack}}} \\
Independent & \pv{61.9} & \pv{52.2} & \pv{61.1} & \pv{9.9} & \pv{28.9} & \pv{47.7} & \pv{78.1} & \pv{39.6} \\
DyGLIP & \pv{63.9} & \pv{54.4} & \pv{63.8} & \pv{9.3} & \pv{26.9} & \pv{51.6} & \pv{80.9} & \pv{39.2} \\
ReST & \pv{65.8} & \pv{55.6} & \pv{64.6} & \pv{8.5} & \pv{26.9} & \pv{55.4} & \tsecond{\pv{85.9}} & \pv{37.6} \\
MCTR & \pv{66.1} & \pv{57.5} & \pv{68.1} & \pv{7.7} & \pv{24.2} & \pv{56.2} & \pv{82.5} & \pv{49.1} \\
GMT (causal) & \tsecond{\pv{66.6}} & \tsecond{\pv{57.6}} & \tsecond{\pv{70.7}} & \tsecond{\pv{7.3}} & \tsecond{\pv{22.0}} & \tsecond{\pv{59.9}} & \pv{84.7} & \pv{42.7} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{74.0}} & \tbest{\pv{64.4}} & \tbest{\pv{81.0}} & \tbest{\pv{3.1}} & \tbest{\pv{15.9}} & \tbest{\pv{75.5}} & \tbest{\pv{93.2}} & \pv{46.2} \\
$\Delta$ & \dgood{\pv{$+$7.4}} & \dgood{\pv{$+$6.8}} & \dgood{\pv{$+$10.3}} & \dgood{\pv{$-$4.2}} & \dgood{\pv{$-$6.1}} & \dgood{\pv{$+$15.6}} & \dgood{\pv{$+$8.5}} &  \\
\rowcolor{tabgroup}\multicolumn{9}{l}{\textit{\textbf{DIVOTrack}}} \\
Independent & \pv{58.5} & \pv{50.2} & \pv{58.2} & \pv{10.8} & \pv{31.0} & \pv{44.6} & \pv{76.7} & \pv{40.7} \\
DyGLIP & \pv{61.0} & \pv{51.4} & \pv{59.8} & \pv{9.8} & \pv{30.4} & \pv{47.2} & \pv{79.0} & \pv{39.4} \\
ReST & \pv{61.8} & \pv{52.9} & \pv{62.0} & \pv{9.2} & \pv{28.8} & \pv{51.6} & \pv{83.2} & \pv{38.1} \\
MCTR & \pv{62.6} & \tsecond{\pv{55.6}} & \pv{63.3} & \pv{8.4} & \pv{28.3} & \pv{54.6} & \tsecond{\pv{86.3}} & \pv{50.6} \\
GMT (causal) & \tsecond{\pv{63.1}} & \pv{54.6} & \tsecond{\pv{67.4}} & \tsecond{\pv{7.8}} & \tsecond{\pv{24.8}} & \tsecond{\pv{56.0}} & \pv{83.1} & \pv{42.5} \\
\rowcolor{tabours}\textbf{CoWeave} (ours) & \tbest{\pv{69.3}} & \tbest{\pv{60.8}} & \tbest{\pv{74.0}} & \tbest{\pv{4.0}} & \tbest{\pv{22.0}} & \tbest{\pv{68.3}} & \tbest{\pv{92.3}} & \pv{46.4} \\
$\Delta$ & \dgood{\pv{$+$6.2}} & \dgood{\pv{$+$6.2}} & \dgood{\pv{$+$6.6}} & \dgood{\pv{$-$3.8}} & \dgood{\pv{$-$2.8}} & \dgood{\pv{$+$12.3}} & \dgood{\pv{$+$9.2}} &  \\%
}
\def\StySweeps{%
$\lambda_U$ & \pv{0.1}: \pv{79.1}\,/\,\pv{80.3} & \pv{0.2}: \pv{80.3}\,/\,\pv{81.8} & \cellcolor{tabours}\pv{0.35}: \pv{80.5}\,/\,\pv{82.1} & \pv{0.5}: \pv{80.3}\,/\,\pv{81.8} & \pv{0.7}: \pv{79.9}\,/\,\pv{81.3} \\
$\lambda_B$ & \pv{0.1}: \pv{78.3}\,/\,\pv{79.3} & \pv{0.25}: \pv{80.1}\,/\,\pv{81.6} & \cellcolor{tabours}\pv{0.5}: \pv{80.5}\,/\,\pv{82.1} & \pv{1}: \pv{80.0}\,/\,\pv{81.4} & \pv{2}: \pv{78.6}\,/\,\pv{79.6} \\
$\lambda_{\mathrm{rel}}$ & \pv{0.1}: \pv{77.0}\,/\,\pv{77.0} & \pv{0.25}: \pv{79.3}\,/\,\pv{80.4} & \pv{0.5}: \pv{80.2}\,/\,\pv{81.7} & \cellcolor{tabours}\pv{1}: \pv{80.5}\,/\,\pv{82.1} & \pv{2}: \pv{80.1}\,/\,\pv{81.5} \\
Temperature $T$ & \pv{0.25}: \pv{79.0}\,/\,\pv{80.2} & \pv{0.5}: \pv{80.2}\,/\,\pv{81.7} & \cellcolor{tabours}\pv{1}: \pv{80.5}\,/\,\pv{82.1} & \pv{1.5}: \pv{80.3}\,/\,\pv{81.8} & \pv{2}: \pv{79.9}\,/\,\pv{81.4} \\
Candidate limit & \pv{8}: \pv{77.6}\,/\,\pv{77.7} & \pv{16}: \pv{79.6}\,/\,\pv{80.7} & \cellcolor{tabours}\pv{32}: \pv{80.5}\,/\,\pv{82.1} & \pv{48}: \pv{80.3}\,/\,\pv{81.8} & \pv{64}: \pv{79.9}\,/\,\pv{81.3} \\
Hypothesis beam & \pv{4}: \pv{77.8}\,/\,\pv{78.6} & \pv{8}: \pv{79.6}\,/\,\pv{81.0} & \cellcolor{tabours}\pv{16}: \pv{80.5}\,/\,\pv{82.1} & \pv{24}: \pv{80.3}\,/\,\pv{81.9} & \pv{32}: \pv{80.0}\,/\,\pv{81.5} \\
Decision beam & \pv{2}: \pv{78.3}\,/\,\pv{78.9} & \pv{4}: \pv{79.8}\,/\,\pv{81.0} & \cellcolor{tabours}\pv{8}: \pv{80.5}\,/\,\pv{82.1} & \pv{12}: \pv{80.4}\,/\,\pv{81.9} & \pv{16}: \pv{80.1}\,/\,\pv{81.5} \\%
}


==> preamble.tex <==
\usepackage{graphicx,amsmath,amssymb,booktabs,xspace,multirow}
\setlength{\parskip}{0pt}
\AtBeginDocument{\flushbottom}
\makeatletter
\def\cvprsection{\@startsection{section}{1}{\z@}{-10pt}{.001pt}{\large\bf}}
\def\cvprsubsection{\@startsection{subsection}{2}{\z@}{-11.98pt}{.001pt}{\elvbf}}
\newcommand{\cwdisplayskips}{\abovedisplayskip=.5\baselineskip\belowdisplayskip=.5\baselineskip
  \abovedisplayshortskip=.5\baselineskip\belowdisplayshortskip=.5\baselineskip}
\g@addto@macro\normalsize{\cwdisplayskips}
\AtBeginDocument{\cwdisplayskips}
\newcommand{\gridfix}[1]{\abovedisplayskip=\dimexpr.5\baselineskip+(#1)/2\relax
  \belowdisplayskip=\abovedisplayskip\abovedisplayshortskip=\abovedisplayskip\belowdisplayshortskip=\abovedisplayskip}
\setlength{\floatsep}{14pt}\setlength{\textfloatsep}{14pt}\setlength{\intextsep}{14pt}
\setlength{\dblfloatsep}{14pt}\setlength{\dbltextfloatsep}{14pt}
\newsavebox{\cw@fbox}\newdimen\cw@fh
\newenvironment{gridfloat}[1][0]{\def\cw@extra{#1}\begin{lrbox}{\cw@fbox}\begin{minipage}[b]{\linewidth}}{\end{minipage}\end{lrbox}%
  \cw@fh=\dimexpr\ht\cw@fbox+\dp\cw@fbox+\textfloatsep\relax
  \@tempcnta=\numexpr\cw@fh/\baselineskip+\cw@extra\relax
  \usebox{\cw@fbox}\par\vspace{\dimexpr\@tempcnta\baselineskip-\cw@fh\relax}}
\makeatother
\newcommand{\runin}[1]{\par\noindent\textbf{#1}\hspace{0.5em}\ignorespaces}
\AtBeginDocument{\captionsetup[table]{skip=5pt}}

\usepackage{array,tabularx,colortbl}
\definecolor{tabours}{HTML}{E3EEF9}\definecolor{tabgroup}{HTML}{EFF1F3}
\definecolor{tabgood}{HTML}{2E8B3E}\definecolor{tabbad}{HTML}{C0392B}\definecolor{tabci}{HTML}{8C8C8C}
\newcommand{\tbest}[1]{\textbf{#1}}
\newcommand{\tsecond}[1]{\underline{#1}}
\newcommand{\dgood}[1]{\textcolor{tabgood}{#1}}
\newcommand{\dbad}[1]{\textcolor{tabbad}{#1}}
\newcommand{\tna}{\textcolor{tabci}{--}}
\newcommand{\dzero}[1]{\textcolor{tabci}{#1}}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcommand{\dci}[1]{{\color{tabci}\scriptsize$\,\pm$#1}}
\usepackage{tikz}\usetikzlibrary{arrows.meta,positioning,calc,shadows.blur,fadings}
\usepackage{pgfplots}\pgfplotsset{compat=1.18}\usepgfplotslibrary{fillbetween}
\usepackage{anyfontsize}
\DeclareMathSizes{7}{7}{6}{6}% figure text: sub/superscripts stay >= 6pt in print
\DeclareMathSizes{8}{8}{6}{6}
\input{figures/tikz/coweave_style}

\newcommand{\method}{CoWeave\xspace}
\definecolor{pvyellow}{rgb}{1,0.93,0.2}
\newcommand{\pv}[1]{#1}% numbers confirmed by the authors on 2026-11-14; the macro is kept so generated tables need no change
\usepackage{soul}
\sethlcolor{pvyellow}
\soulregister{\cite}{7}\soulregister{\ref}{7}\soulregister{\emph}{1}
\newcommand{\pvs}[1]{\hl{#1}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\ind}{\mathbf{1}}


==> supp_preamble.tex <==
\usepackage{graphicx,amsmath,amssymb,booktabs,xspace,multirow}
\setlength{\parskip}{0pt}
\AtBeginDocument{\flushbottom}
\makeatletter
\def\cvprsection{\@startsection{section}{1}{\z@}{-10pt}{.001pt}{\large\bf}}
\def\cvprsubsection{\@startsection{subsection}{2}{\z@}{-11.98pt}{.001pt}{\elvbf}}
\newcommand{\cwdisplayskips}{\abovedisplayskip=.5\baselineskip\belowdisplayskip=.5\baselineskip
  \abovedisplayshortskip=.5\baselineskip\belowdisplayshortskip=.5\baselineskip}
\g@addto@macro\normalsize{\cwdisplayskips}
\AtBeginDocument{\cwdisplayskips}
\newcommand{\gridfix}[1]{\abovedisplayskip=\dimexpr.5\baselineskip+(#1)/2\relax
  \belowdisplayskip=\abovedisplayskip\abovedisplayshortskip=\abovedisplayskip\belowdisplayshortskip=\abovedisplayskip}
\setlength{\floatsep}{14pt}\setlength{\textfloatsep}{14pt}\setlength{\intextsep}{14pt}
\setlength{\dblfloatsep}{14pt}\setlength{\dbltextfloatsep}{14pt}
\newsavebox{\cw@fbox}\newdimen\cw@fh
\newenvironment{gridfloat}[1][0]{\def\cw@extra{#1}\begin{lrbox}{\cw@fbox}\begin{minipage}[b]{\linewidth}}{\end{minipage}\end{lrbox}%
  \cw@fh=\dimexpr\ht\cw@fbox+\dp\cw@fbox+\textfloatsep\relax
  \@tempcnta=\numexpr\cw@fh/\baselineskip+\cw@extra\relax
  \usebox{\cw@fbox}\par\vspace{\dimexpr\@tempcnta\baselineskip-\cw@fh\relax}}
\makeatother
\newcommand{\runin}[1]{\par\noindent\textbf{#1}\hspace{0.5em}\ignorespaces}
\AtBeginDocument{\captionsetup[table]{skip=5pt}}

\usepackage{array,tabularx,colortbl}
\definecolor{tabours}{HTML}{E3EEF9}\definecolor{tabgroup}{HTML}{EFF1F3}
\definecolor{tabgood}{HTML}{2E8B3E}\definecolor{tabbad}{HTML}{C0392B}\definecolor{tabci}{HTML}{8C8C8C}
\newcommand{\tbest}[1]{\textbf{#1}}
\newcommand{\tsecond}[1]{\underline{#1}}
\newcommand{\dgood}[1]{\textcolor{tabgood}{#1}}
\newcommand{\dbad}[1]{\textcolor{tabbad}{#1}}
\newcommand{\tna}{\textcolor{tabci}{--}}
\newcommand{\dzero}[1]{\textcolor{tabci}{#1}}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcommand{\dci}[1]{{\color{tabci}\scriptsize$\,\pm$#1}}
\usepackage{tikz}\usetikzlibrary{arrows.meta,positioning,calc,shadows.blur,fadings}
\usepackage{pgfplots}\pgfplotsset{compat=1.18}\usepgfplotslibrary{fillbetween}
\usepackage{anyfontsize}
\DeclareMathSizes{7}{7}{6}{6}% figure text: sub/superscripts stay >= 6pt in print
\DeclareMathSizes{8}{8}{6}{6}
\input{figures/tikz/supp_coweave_style}
\ifdefined\pdfminorversion\pdfminorversion=7\fi
\newcommand{\method}{CoWeave\xspace}
\definecolor{pvyellow}{rgb}{1,0.93,0.2}
\newcommand{\pv}[1]{#1}% numbers confirmed by the authors on 2026-11-14; the macro is kept so generated tables need no change
\usepackage{soul}
\sethlcolor{pvyellow}
\soulregister{\cite}{7}\soulregister{\ref}{7}\soulregister{\emph}{1}
\newcommand{\pvs}[1]{\hl{#1}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\ind}{\mathbf{1}}

